Validity-Preserving Delta Debugging via Generator Trace Reduction

Reducing test inputs that trigger bugs is crucial for efficient debugging. Delta debugging is the most popular approach for this purpose. When test inputs need to conform to certain specifications, existing delta debugging practice encounters a validity problem: it blindly applies reduction rules, producing a large number of invalid test inputs that do not satisfy the required specifications. This overall diminishing effectiveness and efficiency becomes even more pronounced when the specifications extend beyond syntactical structures. Our key insight is that we should leverage input generators, which are aware of these specifications, to generate valid reduced inputs, rather than straightforwardly performing reduction on test inputs. In this paper, we propose a generator-based delta debugging method, namely GReduce, which derives validity-preserving reducers. Specifically, given a generator and its execution, demonstrating how the bug-inducing test input is generated, GReduce searches for other executions on the generator that yield reduced, valid test inputs. The evaluation results on five benchmarks (i.e., graphs, DL models, JavaScript programs, SymPy, and algebraic data types) show that GReduce substantially outperforms state-of-the-art syntax-based reducers including Perses and T-PDD, and also outperforms QuickCheck, SmartCheck, as well as the state-of-the-art choice-sequence-based reducer Hypothesis, demonstrating the effectiveness, efficiency, and versatility of GReduce.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> sections/newoverview.tex <==

% \subsubsection{Attribute Grammar}
% An attribute grammar (AG) consists of three components: a grammar G, a finite set of attributes A, and a finite set of semantic rules R: $AG = <G, A, R>$.
% G is a quadruple: $G = <N, T, P, D>$, where $N$ is a finite set of \emph{nonterminal symbols}, $T$ is a finite set of \emph{terminal symbols}, $P$ is a finite set of \emph{productions}, and $D \subset N$ is the \emph{start symbol} of $G$. The productions in $P$ are with the form as $X \longrightarrow \alpha$.
% Attributes is associated with each symbol with the form of $X.v=f(y_1,y_2,...y_k)$.


%Given a generator $G$ with a ~\emph{deterministic} input, as well as an interpreter $IntP$, a path $P$ could be derived.


\section{Motivating Examples}\label{sec:s2}
We present two motivating examples to showcase 

\subsection{Effectiveness}

illustrating significant benefits (i.e. effectiveness and efficiency) of reduction on complex test inputs such as DL models via refining the search space of reduction.

% To detect bugs in DL compilers, we rely on generator-based testing, where 

%First, we show a generated test input that triggers a bug. Then, we highlight the difficulties of using existing test input reduction methods (delta debugging algorithms as well as transformation-based reduction) when dealing with complex specifications for test inputs, specifically DL models. Last, we show the effective reduction result of our generator-based reduction.

% We offer a motivating example to demonstrate the clear advantage of our generator-based test input reduction in complex generator-based test scenarios. Our example focuses on testing a deep learning compiler, as the test inputs (DL models) are always generated by a generator with complex input specifications. 
% To detect bugs in DL compilers, we conduct generator-based testing which randomly generates DL models with ensuring its validity by incorporating specification ~\cite{DBLP:journals/corr/abs-2302-00842}\Luyao{cite other generator-based testing for DL Compiler?}.

\subsection{Initial Test Input} 


Suppose the generator produces a test input (a DL model) as shown in Figure~\ref{alg:e1}\footnote{The test input of DL compiler is actually the DL model defined by this program, we show the simplified program instead of model here for brevity.}. This DL model consists of only one operation: 
\CodeIn{Split}~\footnote{\url{https://github.com/onnx/onnx/blob/main/docs/Operators.md\#split}}, as an operation that splits a tensor into a list of tensors, along the specified ‘axis’, also with `split' as lengths of each output. 
This DL model in fact triggers a bug~\footnote{Blind for anonymous review.} related to operation \CodeIn{Split} in our software under testing, which is a popular DL compiler named TVM~\cite{DBLP:conf/osdi/ChenMJZYSCWHCGK18}.

\begin{figure}[htb] 
\begin{algorithmic}[1]
\State $T \gets \Call{InputTensor}{shape = [10]}$
\State $X, Y, Z \gets \Call{Split}{T, sections = [3, 3, 4]}$ 
\end{algorithmic} 
\caption{A generated test input for DL compilers.}
\label{alg:e1} 
\end{figure}


\subsection{Existing Practices on Delta Debugging}

% We first show that the complicated specification of test inputs, i.e., DL models, brings issues for adopting existing test input reduction practice on our example.

Delta Debugging, as the most popular technique, model the test input reduction as a search problem: decomposes the test input $I$ into a set of deltas $D$ ~\cite{ODD} (also named elementary changes in ~\cite{DD}), and applies various delta debugging algorithms (such as \emph{ddmin}~\cite{DD}, HDD~\cite{HDD}, Perses~\cite{Perses}, ProbDD~\cite{ProbDD}) to find a minimum test input~\footnote{
Finding the globally minimal one is usually infeasible since hitting set problem is known to be NP-complete~\cite{DBLP:conf/coco/Karp72}.
Instead, the delta debugging algorithms ensure the reduction result is 1-minimal: if deleting any single element makes the result lose the property.} that still triggers the bug, by iteratively trying candidated test inputs which are composed by subsets of $D$.
% that still exhibits our property (the property in our example is triggering the bug) by iteratively trying candidated test inputs which are composed by subsets of $D$.
%We could indeed straight-forwardly adopting
%, as we named syntax-based test input reduction. 

In our example, followed by existing practices such as \emph{ddmin}~\cite{DD},
%we could straightforwardly adopt delta debugging by decomposing the DL model according to its syntactical structure, following existing delta debugging practice on programs~\cite{HDD, Perses, 10.1145/3586049}.
% However, we will fail on finding a smaller one exhibits the property, due to that our decomposition is based on syntactical structure.
we decompose our example into a sequence $S$ consisting of lines in original test input ~\footnote{It is named line-level decomposition or statement-level decomposition.~\Luyao{add cite?}}: $[L_1,L_2]$ ($L_i$ denotes $i$-th line). Then, delta debugging algorithms iteratively try subsequences of $S$ such as $[L_1]$.

However, we fail to find a reduced test input: including $L_1$ with excluding $L_2$ does not trigger the bug; including $L_2$ but excluding $L_1$ will lead the composed DL model invalid, due to the specification of \CodeIn{Split}, as shown in Figure~\ref{alg:e2}, to say nothing of triggering the bug.

\begin{figure}[htb] 
\begin{algorithmic}[1]
\State \sout{$T \gets \Call{InputTensor}{shape = [10]}$}
\State $X, Y, Z \gets \Call{Split}{T, sections = [3, 3, 4]}$ \Comment{Raise error due to `use-before-define' ($T$ is not existed).}
\end{algorithmic} 
\caption{A candidate of delta debugging based on syntactical structure.}
\label{alg:e2} 
\end{figure}

Other decompositions such as token-level, character-level, and tree-based ones (e.g. HDD~\cite{HDD} and Perses~\cite{Perses}),
%though more finer granularity than line-level one,
face the same situation because none of (proper) syntactic subset of the DL model in Figure~\ref{alg:e1} is valid. As an example, Figure~\ref{alg:e2.2} 

\begin{figure}[htb] 
\begin{algorithmic}[1]
\State $T \gets \Call{InputTensor}{shape = [10]}$
\State $X \mbox{\sout{$, Y, Z $}} \gets \Call{Split}{T, sections = [3,3,4]}$ \Comment{Raise error due to that the number of outputs mismatches the number of sections.}
\end{algorithmic} 
\caption{Another candidate of delta debugging based on syntactical structure.}
\label{alg:e2.2} 
\end{figure}


% it is easy to observe that 

% Even for tree-based decomposition\cite{HDD, Perses}\Luyao{add more}, which requires a parser for test inputs, with more delicate algorithms such as HDD~\cite{HDD} and Perses~\cite{Perses}, also fails for the same reason.

%to finally find minimum result~\footnote{Many of existing DD algorithms target at find a locally minimum one with ensuring 1-minimum~\cite{} instead of globally minimum one.}.





\subsection{Existing Practices on Transformation-based Reduction}
Another technique is transformation-based reduction~\cite{CReduce, 10.1145/3586049}, which iteratively applies transformations on the test input until a global fixpoint is reached. Transformations are usually defined manually by heuristic rules~\cite{CReduce, 10.1145/3586049}, such as identifier replacement~\cite{10.1145/3586049}, i.e., replacing an identifier with another one. For instance, we can replace $T2$ in $L_3$ with $T1$ as shown in Figure~\ref{alg:e3}, which satisfies `use-before-define' specification but unfortunately still violates the specification of \CodeIn{Split} operation~\footnote{\url{https://onnx.ai/onnx/operators/onnx__Split.html\#inputs}}. This is because the length of 1-th dimension of input tensor placeholder (i.e., $4$ of $T1$'s shape $(1,4,8)$) is not equal to the sum of numbers in $split$ (i.e., $32$). %~\Luyao{Transformation still designed based on syntactical structure of test input....}
% However, we could notice that this replacement is the only `successful' one among a lot of alternative replacements, which implies that more transformation may lead to smaller result but probably sacrifice efficiency.
%After that, the test input is able to further remove $Line 2$, produce DL model as Listing~\ref{alg:example2}.

% Compared to delta debugging, fixed-point iteration with transformations, usually regarded as a generalization of delta debugging (because delta debugging could be regarded as working on a single `picking a subset' transformation), 

Although fix-point iteration with transformations have opportunities to obtain a smaller reduced test input by exploring in a larger search space than delta debugging,
%the space of test inputs which could be produced by transformations.
it faces following issues: (1) customizing appropriate transformations requires a significant amount of extra effort, especially for complicated input specification~\cite{CReduce, 10.1145/3586049}. For example, CReduce~\cite{CReduce}, as a domain-specific reducer for C programs, manually design XX~\Luyao{TODO} transformations based on the grammar of C language. (2)
inappropriate transformations will not potentially bring in better results but cost more testing resource due to enlarged search space.
% without bringing in smaller test inputs we are interested in. 
For example, all candidates derived from identifier replacement are invalid in our example\footnote{If it allows continuously apply identifier replacement twice, then few of them will be valid such as swapping $T3$ and $T4$, but no help for reduction.}

% \Luyao{add results of CReduce here, or other?}

% , leading to a waste of testing resource.
%inefficiently search ones that satisfy specification (,

\iffalse

For example, if we would like to reduce the number of outputs for \CodeIn{Split}, we need to customize an ad-hoc transformation such as "simultaneously replacing output $[T_a,T_b,T_c]$ with a subset $[T_b,T_c]$ and replacing $split=[x,y,z]$ with $split=[p, q]$ with satisfying $p+q=x+y+z$ in the meanwhile". 

\fi

% for the effectiveness and efficiency
%As our motivating example shown, existing practices when the test input with specification, the search space is critical for test input reduction: delta debugging with syntactical decomposition/composition is not effective due to a limited search space defined by subsets of test input's syntactical structure;

%Thus, existing test input reduction practices are not directly applicable for our scenario. In order to resolve it, user need to design specific transformation on DL model which costs extra manual effort.However, if this DL model is produced by a generator. We have opportunity to reduce it `for free' via our approach, as we called generator-based test input reduction.


%the space defined in syntax-based test input reduction limits its effectiveness; for transformation-based reduction, fewer transformation limits its effectiveness

%Both of syntax-based and transformation-based test input reduction faces the issue of 
% Obviously, we could achieve global minimum one if we design ad-hoc transformations.


\begin{figure}[htb] 

\begin{algorithmic}[1]
\State $T \gets \Call{InputTensor}{shape = [10]}$
\State $X, Y, \mbox{\sout{$Z$}}T \gets \Call{Split}{T, sections = [3,3,4]}$ \Comment{Raise error due to the redefination.}
\end{algorithmic} 
\caption{A candidate of fixed-point iteration with transformations (via applying identifier replacement)}
\label{alg:e3} 
\end{figure}


\subsection{Generator-based Reduction}

To effectively and efficiently obtain a reduced test input, in contrast to existing practices which explore candidates in the search space derived from the syntactical structure of the test input, \toolname{} refines the search space via generator. Specifically, \toolname{} searches candidates derived from the reduced generation procedure of the test input.

Generation procedure of a test input is defined as a deterministic execution path of a generator~\Luyao{explain more?}, illustrating how the test input is generated. For example, in the design of a DL model generator~\cite{DBLP:journals/corr/abs-2302-00842}, the generation procedure of our example is roughly as follows: first constructs the \CodeIn{Flatten} operation, and then \CodeIn{Split} operation. Note, within the construction of \CodeIn{Split} operation (same as \CodeIn{Flatten}), generator also constructs on its input (i.e., $T2$), output (i.e., $T3, T4, T5$) and other parameters $split$ and $axis$.

\Luyao{TODO}

\iffalse

The key observation behind \toolname{} is that reduction on the generation procedure correlates with~\Luyao{another word?} reduction on the test input.~\Luyao{discussion properties? like monotonicity.}

To conduct reduction on the generation procedure, \toolname{} conducts a technique named $GenDecompose$ to decompose a generation procedure into a data structure, which could be manipulated by existing delta debugging algorithms.

With an interpreter, a generation procedure could be interpreted to a test input.

To build~\Luyao{another word?} the correlation,


Given a generation procedure, \toolname{} conducts two techniques 


searches candidates by conducting delta debugging algorithms 


manipulating on it with the help of three components: (1) $GenDecompose$,


\toolname{} conduct a technique named $GenCompose$ to compose a data structure $D'$ which comes from the manipulation on $D$

with manipulating on generation procedure, we will acquire a test input (i.e., the output of the generator).


To acquire a generation procedure, \toolname{} conduct a technique named $GenDecompose$ which interprets the generator 

It could be acquired by 


 (shown in detail in Section~\ref{sec:s3})

For a given generator
 will decompose 


decompose generator 





with taking the output of \CodeIn{Flatten} as its input. Note, when generator constructs the output of \CodeIn{Split}, it is designed as generating $n - 1$ output(s) first and add the last output by calculating the needed shape for satisfying specification~\cite{DBLP:journals/corr/abs-2302-00842}. This design, as we called incorporated specification, provides \toolname{} with opportunity of reduction without avoid specification.

 (with its input, output and $axis$ parameter); (2)


%In our example, the generation procedure of a DL model generator~\cite{DBLP:journals/corr/abs-2302-00842} is as follows: first construct the \CodeIn{Flatten} operation (with its input, output and $axis$ parameter), then next operation, i.e., \CodeIn{Split}, will be constructed by taking the output of \CodeIn{Flatten} as its input. When generator constructs the output of \CodeIn{Split}, it is designed as generating (n - 1) output(s) first and add the last output by calculating the needed shape for satisfying specification.


The generation procedure of our example contains following 





by three key components as follows


(1) decomposing the generation procedure of the test input into a data structure $D$; (2) composing any substructure of $D$ into a reduced test input; (3) utilizing the existing delta debugging algorithms (i.e., \emph{ddmin} and HDD) to pick some substructures of $D$ and compose 



%decompose the test input by its syntactical structure, \toolname{} decomposes the generation procedure of the test input. Here, 




By decomposes the generation procedure of the test input, as well as compose a subset of generation procedure into the reduced test input.

\Luyao{TODO}
\fi

%Also, with a strategy we called \stwo{}, we could delete the first line and resolving the data dependencies by altering $T2$ as a simpler and invalid one.\Luyao{refine format T2}\Luyao{TODO refine!!}

\begin{figure}[H] 
\small
\begin{algorithmic}[1]
\State $T2 \gets \Call{InputTensor}{shape=[1, 32]}$
\State $T4, T5 \gets \Call{Split}{T2, split = [20, 12], axis = 1}$
\end{algorithmic} 
\caption{The result of generator-based test input reduction.}
\label{alg:e4} 
\end{figure}

We will illustrate our approach in detail in next section.

% \toolname{} decomposes the generation procedure by its control flow as a structure of tree as shown in Figure~\ref{}\Luyao{figure in section 3}, which existing search strategy of DD~\cite{DD} and HDD~\cite{HDD} could be applied on.
% With a technique we named `Interpretation for Reduction', i.e., interpreting the reduced generation procedure with two straightforward\Luyao{concise or simple?} strategies named \sone{} and \stwo{} for resolving data flow dependencies, a reduced generation procedure could compose a smaller and valid DL model  
% as shown in Figure~\ref{alg:e4}.

%which the generation process designed by test developers, 
%Based on our insight of shifting test input reduction space from syntax-based to generator-based, we propose our approach \toolname{} :

%via applying delta debugging algorithms on the generator-based reduction space from 
%`decomposed generator'\Luyao{explain more?}.

%\Luyao{This example shows existing work (syntax-based) is unable to make it smaller on it but GReduce could, thus more effective.This example shows existing work (syntax-based, transformation-based) will easily make it invalid by reduction but GReduce will not, thus more efficient.}




%-------



==> sections/runningexample.tex <==

\begin{lstlisting}[language=Python]
\caption{A generator for DL models\Luyao{refine..}} 


\end{lstlisting}










\begin{figure}[htb] 
\label{alg:alg1} 
\begin{algorithmic}[1]
\Function{genDLModel}{} \Comment{Main function.}
	\State $n \gets$ R.randint(1, MAXOP) \Comment{ n denotes the number of operations in generated DL model.}
    \State $M \gets$ a empty DL model.
    \For{$i = 1$ to $n$}
    \State G.append(\Call{gen\$(Operation)}{}) \Comment{Append a new operation into model.}
    %  (with its inputs, outputs, and other parameters) 
    \EndFor
    \State \Return $M$
\EndFunction

\Function{genFlatten}{}
	\State $I^{Flatten} \gets new Tensor(shape=(d_0, d_1, ..., d_{s-1}))$
        \State $ax \gets  R.randint(1, s-1)$
        \Comment{$ax$ is the dimension of splitting, with incorporating specification that $ax$ should be less than $s$ }
	\State $O^{Flatten} \gets new Tensor(shape=(d_0 * d_1...*d_{ax-1}, d_{ax} * d_{ax+1}...* d_{s-1}))$ \Comment{encodes specification of \CodeIn{Flatten} operation.}
	\State \Return Operation(type=\CodeIn{Flatten}, inputs = $I^{Flatten}$, output = $O^{Flatten}$, $axis=ax$).
\EndFunction

% \Procedure{genMatMul}{}
% 	\State Set a tensor placeholder named $I_1^{MatMul}(x,y)$ \Comment{encodes specification that inputs of \CodeIn{MatMul} should be 2-d tensors}
% 	\State Set a tensor placeholder named $I_2^{MatMul}(y,z)$ \Comment{encodes specification that $I_2^{MatMul} = I_1^{MatMul}$}
% 	\State Set a tensor placeholder named $O^{MatMul}(x,z)$ \Comment{encodes specification that $O^{MatMul}[1] = I_1^{MatMul}[1] \land O^{MatMul}[2] = I_2^{MatMul}[2]$}
% 	\State Create a \CodeIn{MatMul} operation with inputs as $I_1^{MatMul}$, $I_2^{MatMul}$ and output as $O^{MatMul}$; then append it into model.
% \EndProcedure

\Function{genSplit}{}
	\State $I^{Split} \gets new Tensor(shape=(d_0,d_1, ..., d_{t-1}))$
	\State $ax$ as the dimension of splitting \Comment{encodes specification that $ax$ should be an integer in $[0, t)$}
    \State Set  a random integer $L$ as number of outputs \Comment{encodes specification that $L$ should be an integer in  $[1, d_{ax}]$}
	\For{$i = 1$ to $L$}
        \State Set a tensor placeholder named $O_i^{Split}(d_1,...,d_{ax-1},s_i,d_{ax+1}, ..., d_{t-1})$ \Comment{encodes specification of \CodeIn{Split} operation.}%\Comment{encodes specification that $(I^{Split}[ax] = \sum_{k} (O_k^{Split}[ax]) = s_1 + s_2 + ... + s_{L}) \land (\forall_{k,k\neq ax} I^{Split}[k] = O_k^{Split}[k])$}
    \EndFor
    \Return Operation(type=\CodeIn{Split}, inputs = $I^{Split}$, output = $O_1^{Split}, O_2^{Split}, ...,$, $axis=ax$, $sections=[s_1, ..., s_L]$).
    
    %Create a \CodeIn{Split} operation with input as $I^{Split}$, output(s) as $O_1^{Split},...,O_L^{Split}$, and parameters $axis=ax, sections=[s_1, ..., s_L]$; then append it into model.    
\EndFunction

\Function{gen...}{}
\State ...
\EndFunction

\State ...

\caption{A generator for DL models\Luyao{refine..}} 

\end{algorithmic} 
\end{figure}


% \begin{figure}[]
%     \centering
%     \setlength{\abovecaptionskip}{0cm}   
%     \setlength{\belowdisplayskip}{0pt} 
%     \includegraphics[width=\linewidth]{imgs/rp-heng.png}
%     \caption{A Running Example.}
%     \label{fig:runningexample}
% \end{figure}


\iffalse
\begin{algorithm}[h] 
\caption{Procedures of the generator\Luyao{inline gen flatten into.}} 
\label{alg:alg2} 
\begin{algorithmic}[1]
\Procedure{genDLModel}{}	
    %\State $n \gets 2$
    %\For{...}
    \State ...
    \State $P_1$(1-st turn of forloop)$: \Call{genFlatten}{}$
    
    \State $P_2$(2-nd turn of forloop)$: \Call{genSplit}{}$
    \State ...
    %\EndFor
	% \State \Return generated DL model
\EndProcedure


% \Procedure{genMatMul}{}
% 	\State $P_{11}: I_1^{MatMul} \gets TensorPH_1(1,2)$ %\Comment{set $I_1^{MatMul}$ as a tensor placeholder with shape $(1,2)$}
% 	\State $P_{12}: I_2^{MatMul} \gets  TensorPH_2(2,10)$ \Comment{set $I_2^{MatMul}$ as a tensor placeholder with shape $(2,10)$, with encoded specification: $I_2^{MatMul}[1] = I_1^{MatMul}[2] = 2$}
% 	\State $P_{13}: O^{MatMul} \gets TensorPH_3(1, 10)$ 
% 	\State ...
% \EndProcedure

\Procedure{genFlatten}{}
	\State $ P_{11}: I^{Flatten} \gets TensorPH_1(1, 4, 8)$ %\Comment{set $I_1^{MatMul}$ as a tensor placeholder with shape $(1,2)$}
        \State $ P_{12}: ax \gets 1$
	\State $ P_{13}: O^{Flatten} \gets TensorPH_2(1, 32)$ %\Comment{set $I_2^{MatMul}$ as a tensor placeholder with shape $(2,10)$, with encoded specification: $I_2^{MatMul}[1] = I_1^{MatMul}[2] = 2$}
	\State ...
\EndProcedure

\Procedure{genSplit}{}
    \State $P_{21}:I^{Split} \gets O^{Flatten} $ \Comment{set the output of \CodeIn{Flatten} as the input of \CodeIn{Split}, thus shape of $I^{Split}$ is $(1,32)$}
    \State $P_{22}:ax \gets 1$
    \State $P_{23}:L \gets 4$
    \State $P_{231}$(1-st turn of forloop)$: O_1^{Split} \gets TensorPH_3(1,10)$
    \State $P_{232}$(2-nd turn of forloop)$: O_2^{Split} \gets TensorPH_4(1,10)$
    \State $P_{233}$(3-rd turn of forloop)$: O_3^{Split} \gets TensorPH_5(1,I^{Split}[ax]-20)$\Comment{As the last output of \CodeIn{Split}, generator sets the shape of $O_3^{Split}$ with encoded specification: $O_3^{Split}[ax] = I^{Split}[ax] - (O_1^{Split}[ax] + O_2^{Split}[ax] + O_3^{Split}[ax]) = 32 - (10 + 10) = 12$ }
    \State ...
\EndProcedure

\end{algorithmic} 
\end{algorithm}
\fi

\iffalse
\begin{algorithm}[] 
\caption{First turn of \toolname{}} 
\label{alg:alg3} 
\begin{algorithmic}[1]
\Function{genDLModel}{}	
    %\State $n \gets 2$
    %\For{...}
    \State ...
    \State $Mask(P_1) $
    \State $P_2: \Call{genSplit}{}$
    \State ...
    %\EndFor
	% \State \Return generated DL model
\EndFunction
\Procedure{genSplit}{}
    \State ...
\EndProcedure
\end{algorithmic} 
\end{algorithm}
\fi

\begin{algorithm}[] 
\caption{Second turn of \toolname{}} 
\label{alg:alg4} 
\begin{algorithmic}[1]
\Function{genDLModel}{}	
    %\State $n \gets 2$
    %\For{...}
    \State ...
    \State $Mask(P_1) $
    \State $P_2: \Call{genSplit}{}$
    \State ...
    %\EndFor
	% \State \Return generated DL model
\EndFunction


\Procedure{genSplit}{}
	\State $P_{21}': I^{Split} \gets TensorPH_6(1, 32) $ \Comment{\stwo{} strategy: replace $O^{MatMul}$ by a new tensor placeholder with the same shape.\Luyao{think about how to get the shape}}
        \State $P_{22}: ax \gets 1$
	\State ...
    \State $Mask(P_{231})$
    \State $P_{232}: O_2^{Split} \gets TensorPH_4(1,10)$
    \State $P_{233}': O_3^{Split} \gets TensorPH_5(1, 22)$ \Comment{$TensorPH_7[1]$ changes from $12$ to $22$ due to encoded specification (i.e., $O_3^{Split}[1] = I^{Split}[1] - O_2^{Split}[1] = 32 - 12 = 20$)}
    \State ...
\EndProcedure
\end{algorithmic} 

\end{algorithm}




%when the number of operation $Sum$'s input tensor(s) is more than two.

% \begin{figure}[t]
%     \centering
%     \setlength{\abovecaptionskip}{0.2cm}   
%     \setlength{\belowdisplayskip}{0pt} 
%     \includegraphics[width=\linewidth]{imgs/moexample.png}
%     \caption{A real buggy model in TVM v0.7}
%     \label{fig:moexample}
% \end{figure}




==> sections/tmp.tex <==
Consider the task of generating test inputs in language $L$, we conduct a generator written in Python as follows ~\footnote{It is a runnable code under Python 3.8.}:
\begin{lstlisting}[language=Python, caption=A generator G of the language D, label={lst:g0}]
import random as R # set the source of randommness
import string
# R.seed(7257) # uncomment this line for configuring R to deterministically generating "abc\nabc\n"
MAXLEN = 10 # the maximal length of the string
n = R.randint(0, MAXLEN // 2)
for i in range(n):
    s += R.choice(string.ascii_lowercase)
s = s + '\n'
s = s + s
print(s)
\end{lstlisting}




for a deep learning compiler, where we randomly generate DL models while ensuring their validity by incorporating specifications~\cite{DBLP:journals/corr/abs-2302-00842}~\Luyao{mention specifications here?}. 
Suppose the generator produces a test input (a DL model) as shown in Figure~\ref{alg:e1}\footnote{The test input of DL compiler is actually the DL model defined by this program, we show the simplified program instead of model here for brevity.}. This DL model consists of only one operation: 
\CodeIn{Split}~\footnote{\url{https://github.com/onnx/onnx/blob/main/docs/Operators.md\#split}}, as an operation that splits a tensor into a list of tensors, along the specified ‘axis’, also with `split' as lengths of each output. 
This DL model in fact triggers a bug~\footnote{Blind for anonymous review.} related to operation \CodeIn{Split} in our software under testing, which is a popular DL compiler named TVM~\cite{DBLP:conf/osdi/ChenMJZYSCWHCGK18}.

\begin{figure}[htb] 
\begin{algorithmic}[1]
\State $T \gets \Call{InputTensor}{shape = [10]}$
\State $X, Y, Z \gets \Call{Split}{T, sections = [3, 3, 4]}$ 
\end{algorithmic} 
\caption{A generated test input for DL compilers.}
\label{alg:e1} 
\end{figure}


\subsection{Existing Practices on Delta Debugging}

% We first show that the complicated specification of test inputs, i.e., DL models, brings issues for adopting existing test input reduction practice on our example.

Delta Debugging, as the most popular technique, model the test input reduction as a search problem: decomposes the test input $I$ into a set of deltas $D$ ~\cite{ODD} (also named elementary changes in ~\cite{DD}), and applies various delta debugging algorithms (such as \emph{ddmin}~\cite{DD}, HDD~\cite{HDD}, Perses~\cite{Perses}, ProbDD~\cite{ProbDD}) to find a minimum test input~\footnote{
Finding the globally minimal one is usually infeasible since hitting set problem is known to be NP-complete~\cite{DBLP:conf/coco/Karp72}.
Instead, the delta debugging algorithms ensure the reduction result is 1-minimal: if deleting any single element makes the result lose the property.} that still triggers the bug, by iteratively trying candidated test inputs which are composed by subsets of $D$.
% that still exhibits our property (the property in our example is triggering the bug) by iteratively trying candidated test inputs which are composed by subsets of $D$.
%We could indeed straight-forwardly adopting
%, as we named syntax-based test input reduction. 

In our example, followed by existing practices such as \emph{ddmin}~\cite{DD},
%we could straightforwardly adopt delta debugging by decomposing the DL model according to its syntactical structure, following existing delta debugging practice on programs~\cite{HDD, Perses, 10.1145/3586049}.
% However, we will fail on finding a smaller one exhibits the property, due to that our decomposition is based on syntactical structure.
we decompose our example into a sequence $S$ consisting of lines in original test input ~\footnote{It is named line-level decomposition or statement-level decomposition.~\Luyao{add cite?}}: $[L_1,L_2]$ ($L_i$ denotes $i$-th line). Then, delta debugging algorithms iteratively try subsequences of $S$ such as $[L_1]$.

However, we fail to find a reduced test input: including $L_1$ with excluding $L_2$ does not trigger the bug; including $L_2$ but excluding $L_1$ will lead the composed DL model invalid, due to the specification of \CodeIn{Split}, as shown in Figure~\ref{alg:e2}, to say nothing of triggering the bug.

\begin{figure}[htb] 
\begin{algorithmic}[1]
\State \sout{$T \gets \Call{InputTensor}{shape = [10]}$}
\State $X, Y, Z \gets \Call{Split}{T, sections = [4,3,3]}$ \Comment{Raise error due to `use-before-define' ($T$ is not existed).}
\end{algorithmic} 
\caption{A candidate of delta debugging based on syntactical structure.}
\label{alg:e2} 
\end{figure}

Other decompositions such as token-level, character-level, and tree-based ones (e.g. HDD~\cite{HDD} and Perses~\cite{Perses}),
%though more finer granularity than line-level one,
face the same situation because none of (proper) syntactic subset of the DL model in Figure~\ref{alg:e1} is valid. As an example, Figure~\ref{alg:e2.2} 

\begin{figure}[htb] 
\begin{algorithmic}[1]
\State $T \gets \Call{InputTensor}{shape = [10]}$
\State $X \mbox{\sout{$, Y, Z $}} \gets \Call{Split}{T, sections = [3,3,4]}$ \Comment{Raise error due to that the number of outputs mismatches the number of sections.}
\end{algorithmic} 
\caption{Another candidate of delta debugging based on syntactical structure.}
\label{alg:e2.2} 
\end{figure}


% it is easy to observe that 

% Even for tree-based decomposition\cite{HDD, Perses}\Luyao{add more}, which requires a parser for test inputs, with more delicate algorithms such as HDD~\cite{HDD} and Perses~\cite{Perses}, also fails for the same reason.

%to finally find minimum result~\footnote{Many of existing DD algorithms target at find a locally minimum one with ensuring 1-minimum~\cite{} instead of globally minimum one.}.





\subsection{Existing Practices on Transformation-based Reduction}
Another technique is transformation-based reduction~\cite{CReduce, 10.1145/3586049}, which iteratively applies transformations on the test input until a global fixpoint is reached. Transformations are usually defined manually by heuristic rules~\cite{CReduce, 10.1145/3586049}, such as identifier replacement~\cite{10.1145/3586049}, i.e., replacing an identifier with another one. For instance, we can replace $T2$ in $L_3$ with $T1$ as shown in Figure~\ref{alg:e3}, which satisfies `use-before-define' specification but unfortunately still violates the specification of \CodeIn{Split} operation~\footnote{\url{https://onnx.ai/onnx/operators/onnx__Split.html\#inputs}}. This is because the length of 1-th dimension of input tensor placeholder (i.e., $4$ of $T1$'s shape $(1,4,8)$) is not equal to the sum of numbers in $split$ (i.e., $32$). %~\Luyao{Transformation still designed based on syntactical structure of test input....}
% However, we could notice that this replacement is the only `successful' one among a lot of alternative replacements, which implies that more transformation may lead to smaller result but probably sacrifice efficiency.
%After that, the test input is able to further remove $Line 2$, produce DL model as Listing~\ref{alg:example2}.

% Compared to delta debugging, fixed-point iteration with transformations, usually regarded as a generalization of delta debugging (because delta debugging could be regarded as working on a single `picking a subset' transformation), 

Although fix-point iteration with transformations have opportunities to obtain a smaller reduced test input by exploring in a larger search space than delta debugging,
%the space of test inputs which could be produced by transformations.
it faces following issues: (1) customizing appropriate transformations requires a significant amount of extra effort, especially for complicated input specification~\cite{CReduce, 10.1145/3586049}. For example, CReduce~\cite{CReduce}, as a domain-specific reducer for C programs, manually design XX~\Luyao{TODO} transformations based on the grammar of C language. (2)
inappropriate transformations will not potentially bring in better results but cost more testing resource due to enlarged search space.
% without bringing in smaller test inputs we are interested in. 
For example, all candidates derived from identifier replacement are invalid in our example\footnote{If it allows continuously apply identifier replacement twice, then few of them will be valid such as swapping $T3$ and $T4$, but no help for reduction.}

% \Luyao{add results of CReduce here, or other?}

% , leading to a waste of testing resource.
%inefficiently search ones that satisfy specification (,

\iffalse

For example, if we would like to reduce the number of outputs for \CodeIn{Split}, we need to customize an ad-hoc transformation such as "simultaneously replacing output $[T_a,T_b,T_c]$ with a subset $[T_b,T_c]$ and replacing $split=[x,y,z]$ with $split=[p, q]$ with satisfying $p+q=x+y+z$ in the meanwhile". 

\fi

% for the effectiveness and efficiency
%As our motivating example shown, existing practices when the test input with specification, the search space is critical for test input reduction: delta debugging with syntactical decomposition/composition is not effective due to a limited search space defined by subsets of test input's syntactical structure;

%Thus, existing test input reduction practices are not directly applicable for our scenario. In order to resolve it, user need to design specific transformation on DL model which costs extra manual effort.However, if this DL model is produced by a generator. We have opportunity to reduce it `for free' via our approach, as we called generator-based test input reduction.


%the space defined in syntax-based test input reduction limits its effectiveness; for transformation-based reduction, fewer transformation limits its effectiveness

%Both of syntax-based and transformation-based test input reduction faces the issue of 
% Obviously, we could achieve global minimum one if we design ad-hoc transformations.


\begin{figure}[htb] 

\begin{algorithmic}[1]
\State $T \gets \Call{InputTensor}{shape = [10]}$
\State $X, Y, \mbox{\sout{$Z$}}T \gets \Call{Split}{T, sections = [4,3,3]}$ \Comment{Raise error due to the redefination.}
\end{algorithmic} 
\caption{A candidate of fixed-point iteration with transformations (via applying identifier replacement)}
\label{alg:e3} 
\end{figure}


\subsection{Generator-based Reduction}

To effectively and efficiently obtain a reduced test input, in contrast to existing practices which explore candidates in the search space derived from the syntactical structure of the test input, \toolname{} refines the search space via generator. Specifically, \toolname{} searches candidates derived from the reduced generation procedure of the test input.

Generation procedure of a test input is defined as a deterministic execution path of a generator~\Luyao{explain more?}, illustrating how the test input is generated. For example, in the design of a DL model generator~\cite{DBLP:journals/corr/abs-2302-00842}, the generation procedure of our example is roughly as follows: first constructs the \CodeIn{Flatten} operation, and then \CodeIn{Split} operation. Note, within the construction of \CodeIn{Split} operation (same as \CodeIn{Flatten}), generator also constructs on its input (i.e., $T2$), output (i.e., $T3, T4, T5$) and other parameters $split$ and $axis$.

\Luyao{TODO}

\iffalse

The key observation behind \toolname{} is that reduction on the generation procedure correlates with~\Luyao{another word?} reduction on the test input.~\Luyao{discussion properties? like monotonicity.}

To conduct reduction on the generation procedure, \toolname{} conducts a technique named $GenDecompose$ to decompose a generation procedure into a data structure, which could be manipulated by existing delta debugging algorithms.

With an interpreter, a generation procedure could be interpreted to a test input.

To build~\Luyao{another word?} the correlation,


Given a generation procedure, \toolname{} conducts two techniques 


searches candidates by conducting delta debugging algorithms 


manipulating on it with the help of three components: (1) $GenDecompose$,


\toolname{} conduct a technique named $GenCompose$ to compose a data structure $D'$ which comes from the manipulation on $D$

with manipulating on generation procedure, we will acquire a test input (i.e., the output of the generator).


To acquire a generation procedure, \toolname{} conduct a technique named $GenDecompose$ which interprets the generator 

It could be acquired by 


 (shown in detail in Section~\ref{sec:s3})

For a given generator
 will decompose 


decompose generator 





with taking the output of \CodeIn{Flatten} as its input. Note, when generator constructs the output of \CodeIn{Split}, it is designed as generating $n - 1$ output(s) first and add the last output by calculating the needed shape for satisfying specification~\cite{DBLP:journals/corr/abs-2302-00842}. This design, as we called incorporated specification, provides \toolname{} with opportunity of reduction without avoid specification.

 (with its input, output and $axis$ parameter); (2)


%In our example, the generation procedure of a DL model generator~\cite{DBLP:journals/corr/abs-2302-00842} is as follows: first construct the \CodeIn{Flatten} operation (with its input, output and $axis$ parameter), then next operation, i.e., \CodeIn{Split}, will be constructed by taking the output of \CodeIn{Flatten} as its input. When generator constructs the output of \CodeIn{Split}, it is designed as generating (n - 1) output(s) first and add the last output by calculating the needed shape for satisfying specification.


The generation procedure of our example contains following 





by three key components as follows


(1) decomposing the generation procedure of the test input into a data structure $D$; (2) composing any substructure of $D$ into a reduced test input; (3) utilizing the existing delta debugging algorithms (i.e., \emph{ddmin} and HDD) to pick some substructures of $D$ and compose 



%decompose the test input by its syntactical structure, \toolname{} decomposes the generation procedure of the test input. Here, 




By decomposes the generation procedure of the test input, as well as compose a subset of generation procedure into the reduced test input.

\Luyao{TODO}
\fi

%Also, with a strategy we called \stwo{}, we could delete the first line and resolving the data dependencies by altering $T2$ as a simpler and invalid one.\Luyao{refine format T2}\Luyao{TODO refine!!}

\begin{figure}[H] 
\begin{algorithmic}[1]
\State $T2 \gets \Call{InputTensor}{shape=[10]}$
\State $T4, T5 \gets \Call{Split}{T2, split = [3, 7], axis = 1}$
\end{algorithmic} 
\caption{The result of generator-based test input reduction.}
\label{alg:e4} 
\end{figure}

We will illustrate our approach in detail in next section.

% \toolname{} decomposes the generation procedure by its control flow as a structure of tree as shown in Figure~\ref{}\Luyao{figure in section 3}, which existing search strategy of DD~\cite{DD} and HDD~\cite{HDD} could be applied on.
% With a technique we named `Interpretation for Reduction', i.e., interpreting the reduced generation procedure with two straightforward\Luyao{concise or simple?} strategies named \sone{} and \stwo{} for resolving data flow dependencies, a reduced generation procedure could compose a smaller and valid DL model  
% as shown in Figure~\ref{alg:e4}.

%which the generation process designed by test developers, 
%Based on our insight of shifting test input reduction space from syntax-based to generator-based, we propose our approach \toolname{} :

%via applying delta debugging algorithms on the generator-based reduction space from 
%`decomposed generator'\Luyao{explain more?}.

%\Luyao{This example shows existing work (syntax-based) is unable to make it smaller on it but GReduce could, thus more effective.This example shows existing work (syntax-based, transformation-based) will easily make it invalid by reduction but GReduce will not, thus more efficient.}




%-------


==> tables/figs.tex <==
\begin{figure}[H]
\centering
\subfigure[1]{
%\label{time.1}
\includegraphics[]{imgs/S_G.pdf}}
\quad
\subfigure[2]{
%\label{time.2}
\includegraphics[]{imgs/S_DL.pdf}
\quad
\subfigure[3]{
%\label{time.2}
\includegraphics[]{imgs/S_js.pdf}
}
\caption{Statistical results of different approaches on reduction quality (\redq}
\label{fig:size}
\end{figure}


% \begin{figure*}[h]
%     \centering
%     \resizebox{
%         \textwidth}{!}{\includegraphics{tables/fsize.png}
%     }
%     \caption{Statistical results of different approaches on reduction quality (\redq)}
%     \label{fig:size}
%     \vspace{-0.5cm}
% \end{figure*}
% % \vspace*{-\baselineskip}

% \begin{figure*}[h]
%     \centering
%     \resizebox{\textwidth}{!}{\includegraphics{tables/ftime.png}}
%     \caption{Statistical results of different approaches in reduction time ($Time$).}
%     \label{fig:time}
% \end{figure*}
% % \vspace*{-\baselineskip}



==> tables/t1.tex <==
% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%           & our-candidates & our-time & our-output-size & baseline \\ \hline
% jgrapht-1 &                &          &                 &          \\ \hline
% jgrapht-2 &                &          &                 &          \\ \hline
% js-1      &                &          &                 &          \\ \hline
% \end{tabular}
% \end{table*}

\begin{figure*}[]
    \centering
    \setlength{\abovecaptionskip}{0cm}   
    \setlength{\belowdisplayskip}{0pt} 
    \includegraphics[width=\linewidth]{imgs/result.png}
    \caption{Result.}
    \label{fig:result}
\end{figure*}


==> tables/t1_another.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[h]\scriptsize
\centering
\caption{Detailed Data of Experiment Result (* Denotes Timeout)}
\label{experiment_result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
\hline
\multicolumn{1}{c}{}                   & \multicolumn{1}{c}{}                        & \multicolumn{3}{c}{$GReduce_{r}$}                                                                                                 & \multicolumn{3}{c}{$Greduce^{S}_{b}$}                                                                                            & \multicolumn{3}{c}{$Greduce^{S}_{a}$}                                                                                           & \multicolumn{3}{c}{$Greduce^{T}_{b}$}                                                                                           & \multicolumn{3}{c}{$Greduce^{T}_{a}$}                                                                                           & \multicolumn{3}{c}{$Perses$}                                                                                                      & \multicolumn{3}{c}{$JSDelta$}                                                                                            \\
\multicolumn{1}{c}{\multirow{-2}{*}{}} & \multicolumn{1}{c}{\multirow{-2}{*}{$S_{o}$}} & \textbf{S}           & \textbf{T}     &\textbf{P}      & \textbf{S}           & \textbf{T}     &\textbf{P}     & \textbf{S}           & \textbf{T}    &\textbf{P}     & \textbf{S}           & \textbf{T}    &\textbf{P}     & \textbf{S}          & \textbf{T}     &\textbf{P}     & \textbf{S}          & \textbf{T}      &\textbf{P}      & \textbf{S}    & \textbf{T}    &\textbf{P}    \\ \hline
G-1                                    & (100, 500)                                  & (2, 1)               & 74.6           &147             & (2, 1)               & 18             &24             & (2, 1)               & 15.9          &43             & (2, 1)               & 12.4          &43             & (2, 1)              & 13.1           &24             & (2, 1)              & 102.4           &1929            & -             & -             &-             \\
G-2                                    & (100, 150)                                  & (3, 2)               & 172.4          &292             & (3, 2)               & 73.6           &41             & (3, 2)               & 112.7         &75             & (3, 2)               & 48.2          &72             & (3, 2)              & 71.1           &37             & (3, 2)              & 90.6            &921             & -             & -             &-             \\
G-3                                    & (100, 150)                                  & (15, 14)             & 466.5          &1500            & (9, 8)               & 180.8          &100            & (6, 5)               & 114.7         &309            & (7, 6)               & 58.2          &173            & (5, 4)              & 91.9           &74             & (9, 8)              & 188.1           &1208            & -             & -             &-             \\
G-4                                    & (100, 500)                                  & (3, 9)               & 718.2          &1124            & (3, 9)               & 172.6          &58             & (3, 4)               & 207.6         &129            & (3, 8)               & 89            &121            & (3, 5)              & 96.3           &50             & (65, 19)            & 1322.5          &3312            & -             & -             &-             \\
G-5                                    & (100, 500)                                  & (2, 0)               & 5              &15              & (2, 0)               & 5.1            &10             & (2, 1)               & 27.4          &12             & (2, 0)               & 3.3           &43             & (2, 1)              & 24.6           &19             & (2, 1)              & 81.3            &1929            & -             & -             &-             \\
G-6                                    & (100, 150)                                  & (41, 50)             & 2517.5         &4273            & (26, 32)             & 1332.1         &408            & (24, 31)             & 1261.8        &982            & (23, 31)             & 606.7         &899            & (14, 21)            & 400.4          &262            & (35, 44)            & 975.2           &2643            & -             & -             &-             \\
G-7                                    & (20, 380)                                   & (20, 22)             & 409            &703             & (20, 21)             & 290.7          &55             & (12, 13)             & 414.7         &626            & (4, 5)               & 53.7          &549            & (12, 13)            & 170.6          &246            & (20, 21)            & 369.8           &2132            & -             & -             &-             \\
G-8                                    & (100, 500)                                  & (52, 55)             & 3037.6         &5925            & (44, 47)             & 2142           &199            & (21, 21)             & 1362          &2427           & (6, 6)               & 145           &1216           & (5, 5)              & 140.3          &100            & (53, 56)            & 793.3           &4090            & -             & -             &-             \\
G-9                                    & (100, 500)                                  & (15, 15)             & 1324.8         &1897            & (15, 15)             & 711.6          &99             & (12, 12)             & 559.8         &603            & (7, 7)               & 214.4         &479            & (6, 6)              & 279.5          &110            & (19, 19)            & 455.2           &2681            & -             & -             &-             \\
G-10                                   & (100, 500)                                  & (17, 17)             & 865.7          &1885            & (15, 15)             & 384.4          &110            & (9, 9)               & 463.7         &753            & (5, 5)               & 69.6          &489            & (5, 5)              & 164.4          &139            & (12, 12)            & 277.9           &2409            & -             & -             &-             \\
\textbf{Avg.}                              & \textbf{(92, 383)}                          & \textbf{(17, 18.5)}  & \textbf{959.1} &\textbf{1776.1} & \textbf{(13.9, 15)}  & \textbf{531.1} &\textbf{110.4} & \textbf{(9.4, 9.9)}  & \textbf{454}  &\textbf{595.9} & \textbf{(6.2, 7.1)}  & \textbf{130}  &\textbf{408.4} & \textbf{(5.7, 6.3)} & \textbf{145.2} &\textbf{106.1} & \textbf{(22, 18.3)} & \textbf{465.6}  &\textbf{2325.4} & \textbf{-}    & \textbf{-}    &\textbf{-}    \\ \hline
DL-1                                   & (67, 113)                                   & (58, 99)             & 1.4            &9               & (10, 13)             & 5.8            &33             & (10, 13)             & 2.5           &48             & (10, 13)             & 2.5           &48             & (10, 13)            & 2              &33             & (22, 32)            & 3600*            &9547            & -             & -             &-             \\
DL-2                                   & (59, 97)                                    & (58, 95)             & 1.3            &28              & (15, 27)             & 95.5           &97             & (11, 19)             & 45.6          &106            & (15, 27)             & 80.3          &68             & (11, 19)            & 79.8           &75             & (17, 31)            & 3600*            &7931            & -             & -             &-             \\
DL-3                                   & (101, 185)                                  & (94, 158)            & 4.7            &53              & (6, 9)               & 10.3           &30             & (6, 9)               & 41.6          &42             & (6, 9)               & 7.8           &42             & (6, 9)              & 26             &30             & (12, 22)            & 3600*            &8434            & -             & -             &-             \\
DL-4                                   & (47, 85)                                    & (45, 77)             & 1              &18              & (9, 14)              & 15.4           &41             & (7, 11)              & 25.9          &43             & (9, 14)              & 15.3          &38             & (7, 11)             & 19.7           &32             & (18, 33)            & 3600*            &7650            & -             & -             &-             \\
DL-5                                   & (35, 55)                                    & (29, 48)             & 0.8            &7               & (11, 19)             & 29             &62             & (8, 13)              & 37.5          &65             & (11, 19)             & 33.7          &35             & (8, 13)             & 34.5           &36             & (11, 19)            & 3600*            &7824            & -             & -             &-             \\
DL-6                                   & (126, 246)                                  & (124, 234)           & 3.3            &13              & (19, 35)             & 39.4           &114            & (7, 12)              & 2.7           &134            & (20, 36)             & 50.5          &45             & (8, 13)             & 2.4            &40             & (25, 46)            & 3600*            &6946            & -             & -             &-             \\
DL-7                                   & (108, 207)                                  & (106, 189)           & 3.4            &12              & (10, 16)             & 28.3           &70             & (6, 9)               & 26.6          &67             & (10, 16)             & 31.6          &40             & (6, 9)              & 24.7           &32             & (28, 42)            & 2377            &4767            & -             & -             &-             \\
DL-8                                   & (45, 105)                                   & (39, 75)             & 1.5            &13              & (8, 15)              & 13.5           &41             & (6, 10)              & 21.4          &72             & (9, 17)              & 7.2           &38             & (6, 10)             & 13.1           &25             & (8, 14)             & 2680            &6154            & -             & -             &-             \\
DL-9                                   & (99, 203)                                   & (94, 166)            & 3.5            &18              & (10, 16)             & 9.4            &41             & (9, 16)              & 13            &44             & (10, 16)             & 10.8          &46             & (10, 16)            & 9.8            &37             & (17, 26)            & 3600*            &7515            & -             & -             &-             \\
DL-10                                  & (117, 255)                                  & (107, 206)           & 9.9            &73              & (5, 9)               & 11.1           &44             & (5, 7)               & 28.3          &40             & (5, 9)               & 13.7          &42             & (5, 7)              & 27.7           &44             & (13, 25)            & 3600*            &7202            & -             & -             &-             \\
DL-11                                  & (54, 89)                                    & (51, 84)             & 0.8            &5               & (10, 18)             & 20.5           &68             & (5, 9)               & 10.1          &87             & (10, 19)             & 29.1          &37             & (5, 10)             & 4.7            &16             & (16, 29)            & 3600*            &6587            & -             & -             &-             \\
DL-12                                  & (114, 229)                                  & (111, 204)           & 4.3            &27              & (5, 8)               & 12.6           &41             & (10, 18)             & 24.1          &42             & (5, 8)               & 15.2          &66             & (2, 2)              & 1.1            &11             & (32, 59)            & 3600*            &7844            & -             & -             &-             \\
DL-13                                  & (94, 171)                                   & (86, 150)            & 2.6            &12              & (17, 34)             & 28.3           &59             & (9, 17)              & 30.2          &167            & (15, 28)             & 7.6           &61             & (5, 7)              & 3.4            &12             & (19, 31)            & 3600*            &8400            & -             & -             &-             \\
DL-14                                  & (53, 109)                                   & (52, 106)            & 1.1            &6               & (10, 18)             & 31.2           &71             & (7, 13)              & 45.4          &78             & (10, 18)             & 46.7          &60             & (7, 13)             & 37             &57             & (15, 30)            & 3600*            &7684            & -             & -             &-             \\
DL-15                                  & (114, 202)                                  & (110, 187)           & 2.6            &31              & (6, 10)              & 5              &27             & (4, 6)               & 1.4           &38             & (6, 10)              & 2.5           &26             & (4, 6)              & 0.9            &20             & (16, 30)            & 3600*            &7881            & -             & -             &-             \\
DL-16                                  & (110, 184)                                  & (105, 172)           & 2.4            &34              & (11, 17)             & 2.9            &23             & (10, 15)             & 3             &31             & (11, 17)             & 2.8           &29             & (10, 15)            & 1.5            &21             & (12, 19)            & 3600*            &8172            & -             & -             &-             \\
DL-17                                  & (90, 165)                                   & (88, 149)            & 2              &30              & (6, 13)              & 4.7            &29             & (5, 11)              & 11.2          &60             & (6, 14)              & 2.9           &48             & (5, 12)             & 5.5            &26             & (8, 15)             & 2646            &6107            & -             & -             &-             \\
DL-18                                  & (44, 92)                                    & (42, 79)             & 0.8            &19              & (12, 20)             & 21.2           &73             & (3, 3)               & 0.2           &69             & (12, 20)             & 26.7          &8              & (3, 3)              & 0.8            &10             & (18, 30)            & 1761            &3985            & -             & -             &-             \\
DL-19                                  & (128, 244)                                  & (125, 209)           & 3.2            &24              & (3, 3)               & 0.6            &12             & (3, 3)               & 0.7           &14             & (3, 3)               & 0.5           &12             & (3, 3)              & 1.3            &12             & (5, 5)              & 2608            &5433            & -             & -             &-             \\
DL-20                                  & (80, 164)                                   & (75, 131)            & 1.4            &17              & (6, 9)               & 15.3           &21             & (3, 3)               & 0.3           &32             & (6, 9)               & 8.8           &11             & (3, 3)              & 0.2            &9              & (27, 42)            & 3600*            &7775            & -             & -             &-             \\
\textbf{Avg.}                              & \textbf{(84.3, 160)}                        & \textbf{(80, 140.9)} & \textbf{2.6}   &\textbf{22.5}   & \textbf{(9.5, 16.2)} & \textbf{20}    &\textbf{49.9}  & \textbf{(6.7, 10.9)} & \textbf{18.6} &\textbf{64}    & \textbf{(9.5, 16.1)} & \textbf{19.8} &\textbf{40}    & \textbf{(6.2, 9.7)} & \textbf{14.8}  &\textbf{28.9}  & \textbf{(17, 29)}   & \textbf{3303.6} &\textbf{7191.9} & \textbf{-}    & \textbf{-}    &\textbf{-}    \\ \hline
JS-1                                   & 134                                         & 64                   & 72             &114             & 83                   & 141.5          &172            & 20                   & 35.4          &351            & 86                   & 79.9          &73             & 20                  & 23.6           &40             & 25                  & 16.5            &30              & 34            & 2.1           &4             \\
JS-2                                   & 508                                         & 170                  & 505.2          &686             & 142                  & 236.8          &178            & 70                   & 143.5         &414            & 146                  & 115.4         &268            & 64                  & 52.9           &86             & 86                  & 80.5            &125             & 97            & 28.9          &47            \\
JS-3                                   & 182                                         & 34                   & 66.9           &114             & 20                   & 42.4           &40             & 11                   & 29            &76             & 20                   & 24.6          &54             & 19                  & 19.4           &33             & 15                  & 14.6            &26              & 15            & 11.7          &19            \\
JS-4                                   & 264                                         & 33                   & 44.5           &78              & 34                   & 86.2           &82             & 7                    & 57.6          &192            & 34                   & 39.5          &118            & 7                   & 15.8           &29             & 18                  & 22.4            &41              & 25            & 7.6           &12            \\
JS-5                                   & 347                                         & 81                   & 115.3          &185             & 57                   & 140.3          &73             & 43                   & 125.3         &242            & 66                   & 47            &207            & 43                  & 26.9           &43             & 52                  & 44.2            &81              & 38            & 31.7          &47            \\
JS-6                                   & 131                                         & 41                   & 42.6           &74              & 34                   & 60.6           &34             & 17                   & 41.7          &99             & 34                   & 21.7          &76             & 19                  & 17.4           &28             & 27                  & 21.9            &38              & 36            & 12.4          &21            \\
JS-7                                   & 246                                         & 40                   & 36.8           &64              & 24                   & 63.4           &51             & 13                   & 50.6          &122            & 24                   & 27.9          &107            & 13                  & 15.2           &28             & 19                  & 23.5            &43              & 30            & 9.6           &17            \\
JS-8                                   & 549                                         & 134                  & 175.6          &298             & 131                  & 433.8          &310            & 77                   & 208.8         &694            & 163                  & 165.1         &347            & 103                 & 87.8           &136            & 102                 & 73.5            &128             & 103           & 28.6          &45            \\
JS-9                                   & 144                                         & 20                   & 10.5           &20              & 19                   & 76             &311            & 7                    & 41.5          &104            & 23                   & 22.4          &73             & 7                   & 10.7           &20             & 13                  & 7.6             &14              & 36            & 3.8           &7             \\
JS-10                                  & 569                                         & 28                   & 18.3           &34              & 12                   & 93.5           &312            & 12                   & 55.3          &100            & 12                   & 11.8          &100            & 12                  & 11.4           &20             & 12                  & 12              &23              & 13            & 8.4           &15            \\
\textbf{Avg.}                              & \textbf{307.4}                              & \textbf{64.5}        & \textbf{108.8} &\textbf{166.7}  & \textbf{55.6}        & \textbf{137.5} &\textbf{156.3} & \textbf{27.7}        & \textbf{78.9} &\textbf{239.4} & \textbf{60.8}        & \textbf{55.5} &\textbf{142.3} & \textbf{30.7}       & \textbf{28.1}  &\textbf{46.3}  & \textbf{36.9}       & \textbf{31.7}   &\textbf{54.9}   & \textbf{42.7} & \textbf{14.5} &\textbf{23.4} \\ \hline
\end{tabular}%
}
\end{table*}



==> tables/t1_big.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[h]\scriptsize
\centering
\caption{Detailed Data of Experiment Result (* Denotes Timeout)}
\label{experiment_result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
\hline
\multicolumn{1}{c}{}                   & \multicolumn{1}{c}{}                        & \multicolumn{3}{c}{$GReduce_{r}$}                                                                                                 & \multicolumn{3}{c}{$Greduce^{S}_{b}$}                                                                                            & \multicolumn{3}{c}{$Greduce^{S}_{a}$}                                                                                           & \multicolumn{3}{c}{$Greduce^{T}_{b}$}                                                                                           & \multicolumn{3}{c}{$Greduce^{T}_{a}$}                                                                                           & \multicolumn{3}{c}{$Perses$}                                                                                                      & \multicolumn{3}{c}{$JSDelta$}                                                                                            \\
\multicolumn{1}{c}{\multirow{-2}{*}{}} & \multicolumn{1}{c}{\multirow{-2}{*}{$S_{o}$}} & \cellcolor[HTML]{F8CBAD}\textbf{S}           & \cellcolor[HTML]{FFE699}\textbf{T}     & \cellcolor[HTML]{D5F1A9}\textbf{P}      & \cellcolor[HTML]{F9CCAD}\textbf{S}           & \cellcolor[HTML]{FFE699}\textbf{T}     & \cellcolor[HTML]{D5F1A9}\textbf{P}     & \cellcolor[HTML]{F9CCAD}\textbf{S}           & \cellcolor[HTML]{FFE699}\textbf{T}    & \cellcolor[HTML]{D5F1A9}\textbf{P}     & \cellcolor[HTML]{F9CCAD}\textbf{S}           & \cellcolor[HTML]{FFE699}\textbf{T}    & \cellcolor[HTML]{D5F1A9}\textbf{P}     & \cellcolor[HTML]{F9CCAD}\textbf{S}          & \cellcolor[HTML]{FFE699}\textbf{T}     & \cellcolor[HTML]{D5F1A9}\textbf{P}     & \cellcolor[HTML]{F9CCAD}\textbf{S}          & \cellcolor[HTML]{FFE699}\textbf{T}      & \cellcolor[HTML]{D5F1A9}\textbf{P}      & \cellcolor[HTML]{F9CCAD}\textbf{S}    & \cellcolor[HTML]{FFE699}\textbf{T}    & \cellcolor[HTML]{D5F1A9}\textbf{P}    \\ \hline
G-1                                    & (100, 500)                                  & \cellcolor[HTML]{F8CBAD}(2, 1)               & \cellcolor[HTML]{FFE699}74.6           & \cellcolor[HTML]{D5F1A9}147             & \cellcolor[HTML]{F9CCAD}(2, 1)               & \cellcolor[HTML]{FFE699}18             & \cellcolor[HTML]{D5F1A9}24             & \cellcolor[HTML]{F9CCAD}(2, 1)               & \cellcolor[HTML]{FFE699}15.9          & \cellcolor[HTML]{D5F1A9}43             & \cellcolor[HTML]{F9CCAD}(2, 1)               & \cellcolor[HTML]{FFE699}12.4          & \cellcolor[HTML]{D5F1A9}43             & \cellcolor[HTML]{F9CCAD}(2, 1)              & \cellcolor[HTML]{FFE699}13.1           & \cellcolor[HTML]{D5F1A9}24             & \cellcolor[HTML]{F9CCAD}(2, 1)              & \cellcolor[HTML]{FFE699}102.4           & \cellcolor[HTML]{D5F1A9}1929            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-2                                    & (100, 150)                                  & \cellcolor[HTML]{F9CCAD}(3, 2)               & \cellcolor[HTML]{FFE699}172.4          & \cellcolor[HTML]{D5F1A9}292             & \cellcolor[HTML]{F9CCAD}(3, 2)               & \cellcolor[HTML]{FFE699}73.6           & \cellcolor[HTML]{D5F1A9}41             & \cellcolor[HTML]{F9CCAD}(3, 2)               & \cellcolor[HTML]{FFE699}112.7         & \cellcolor[HTML]{D5F1A9}75             & \cellcolor[HTML]{F9CCAD}(3, 2)               & \cellcolor[HTML]{FFE699}48.2          & \cellcolor[HTML]{D5F1A9}72             & \cellcolor[HTML]{F9CCAD}(3, 2)              & \cellcolor[HTML]{FFE699}71.1           & \cellcolor[HTML]{D5F1A9}37             & \cellcolor[HTML]{F9CCAD}(3, 2)              & \cellcolor[HTML]{FFE699}90.6            & \cellcolor[HTML]{D5F1A9}921             & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-3                                    & (100, 150)                                  & \cellcolor[HTML]{F8CBAD}(15, 14)             & \cellcolor[HTML]{FFE699}466.5          & \cellcolor[HTML]{D5F1A9}1500            & \cellcolor[HTML]{F9CCAD}(9, 8)               & \cellcolor[HTML]{FFE699}180.8          & \cellcolor[HTML]{D5F1A9}100            & \cellcolor[HTML]{F9CCAD}(6, 5)               & \cellcolor[HTML]{FFE699}114.7         & \cellcolor[HTML]{D5F1A9}309            & \cellcolor[HTML]{F9CCAD}(7, 6)               & \cellcolor[HTML]{FFE699}58.2          & \cellcolor[HTML]{D5F1A9}173            & \cellcolor[HTML]{F9CCAD}(5, 4)              & \cellcolor[HTML]{FFE699}91.9           & \cellcolor[HTML]{D5F1A9}74             & \cellcolor[HTML]{F9CCAD}(9, 8)              & \cellcolor[HTML]{FFE699}188.1           & \cellcolor[HTML]{D5F1A9}1208            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-4                                    & (100, 500)                                  & \cellcolor[HTML]{F8CBAD}(3, 9)               & \cellcolor[HTML]{FFE699}718.2          & \cellcolor[HTML]{D5F1A9}1124            & \cellcolor[HTML]{F9CCAD}(3, 9)               & \cellcolor[HTML]{FFE699}172.6          & \cellcolor[HTML]{D5F1A9}58             & \cellcolor[HTML]{F9CCAD}(3, 4)               & \cellcolor[HTML]{FFE699}207.6         & \cellcolor[HTML]{D5F1A9}129            & \cellcolor[HTML]{F9CCAD}(3, 8)               & \cellcolor[HTML]{FFE699}89            & \cellcolor[HTML]{D5F1A9}121            & \cellcolor[HTML]{F9CCAD}(3, 5)              & \cellcolor[HTML]{FFE699}96.3           & \cellcolor[HTML]{D5F1A9}50             & \cellcolor[HTML]{F9CCAD}(65, 19)            & \cellcolor[HTML]{FFE699}1322.5          & \cellcolor[HTML]{D5F1A9}3312            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-5                                    & (100, 500)                                  & \cellcolor[HTML]{F8CBAD}(2, 0)               & \cellcolor[HTML]{FFE699}5              & \cellcolor[HTML]{D5F1A9}15              & \cellcolor[HTML]{F9CCAD}(2, 0)               & \cellcolor[HTML]{FFE699}5.1            & \cellcolor[HTML]{D5F1A9}10             & \cellcolor[HTML]{F9CCAD}(2, 1)               & \cellcolor[HTML]{FFE699}27.4          & \cellcolor[HTML]{D5F1A9}12             & \cellcolor[HTML]{F9CCAD}(2, 0)               & \cellcolor[HTML]{FFE699}3.3           & \cellcolor[HTML]{D5F1A9}43             & \cellcolor[HTML]{F9CCAD}(2, 1)              & \cellcolor[HTML]{FFE699}24.6           & \cellcolor[HTML]{D5F1A9}19             & \cellcolor[HTML]{F9CCAD}(2, 1)              & \cellcolor[HTML]{FFE699}81.3            & \cellcolor[HTML]{D5F1A9}1929            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-6                                    & (100, 150)                                  & \cellcolor[HTML]{F8CBAD}(41, 50)             & \cellcolor[HTML]{FFE699}2517.5         & \cellcolor[HTML]{D5F1A9}4273            & \cellcolor[HTML]{F9CCAD}(26, 32)             & \cellcolor[HTML]{FFE699}1332.1         & \cellcolor[HTML]{D5F1A9}408            & \cellcolor[HTML]{F9CCAD}(24, 31)             & \cellcolor[HTML]{FFE699}1261.8        & \cellcolor[HTML]{D5F1A9}982            & \cellcolor[HTML]{F9CCAD}(23, 31)             & \cellcolor[HTML]{FFE699}606.7         & \cellcolor[HTML]{D5F1A9}899            & \cellcolor[HTML]{F9CCAD}(14, 21)            & \cellcolor[HTML]{FFE699}400.4          & \cellcolor[HTML]{D5F1A9}262            & \cellcolor[HTML]{F9CCAD}(35, 44)            & \cellcolor[HTML]{FFE699}975.2           & \cellcolor[HTML]{D5F1A9}2643            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-7                                    & (20, 380)                                   & \cellcolor[HTML]{F8CBAD}(20, 22)             & \cellcolor[HTML]{FFE699}409            & \cellcolor[HTML]{D5F1A9}703             & \cellcolor[HTML]{F9CCAD}(20, 21)             & \cellcolor[HTML]{FFE699}290.7          & \cellcolor[HTML]{D5F1A9}55             & \cellcolor[HTML]{F9CCAD}(12, 13)             & \cellcolor[HTML]{FFE699}414.7         & \cellcolor[HTML]{D5F1A9}626            & \cellcolor[HTML]{F9CCAD}(4, 5)               & \cellcolor[HTML]{FFE699}53.7          & \cellcolor[HTML]{D5F1A9}549            & \cellcolor[HTML]{F9CCAD}(12, 13)            & \cellcolor[HTML]{FFE699}170.6          & \cellcolor[HTML]{D5F1A9}246            & \cellcolor[HTML]{F9CCAD}(20, 21)            & \cellcolor[HTML]{FFE699}369.8           & \cellcolor[HTML]{D5F1A9}2132            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-8                                    & (100, 500)                                  & \cellcolor[HTML]{F8CBAD}(52, 55)             & \cellcolor[HTML]{FFE699}3037.6         & \cellcolor[HTML]{D5F1A9}5925            & \cellcolor[HTML]{F9CCAD}(44, 47)             & \cellcolor[HTML]{FFE699}2142           & \cellcolor[HTML]{D5F1A9}199            & \cellcolor[HTML]{F9CCAD}(21, 21)             & \cellcolor[HTML]{FFE699}1362          & \cellcolor[HTML]{D5F1A9}2427           & \cellcolor[HTML]{F9CCAD}(6, 6)               & \cellcolor[HTML]{FFE699}145           & \cellcolor[HTML]{D5F1A9}1216           & \cellcolor[HTML]{F9CCAD}(5, 5)              & \cellcolor[HTML]{FFE699}140.3          & \cellcolor[HTML]{D5F1A9}100            & \cellcolor[HTML]{F9CCAD}(53, 56)            & \cellcolor[HTML]{FFE699}793.3           & \cellcolor[HTML]{D5F1A9}4090            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-9                                    & (100, 500)                                  & \cellcolor[HTML]{F8CBAD}(15, 15)             & \cellcolor[HTML]{FFE699}1324.8         & \cellcolor[HTML]{D5F1A9}1897            & \cellcolor[HTML]{F9CCAD}(15, 15)             & \cellcolor[HTML]{FFE699}711.6          & \cellcolor[HTML]{D5F1A9}99             & \cellcolor[HTML]{F9CCAD}(12, 12)             & \cellcolor[HTML]{FFE699}559.8         & \cellcolor[HTML]{D5F1A9}603            & \cellcolor[HTML]{F9CCAD}(7, 7)               & \cellcolor[HTML]{FFE699}214.4         & \cellcolor[HTML]{D5F1A9}479            & \cellcolor[HTML]{F9CCAD}(6, 6)              & \cellcolor[HTML]{FFE699}279.5          & \cellcolor[HTML]{D5F1A9}110            & \cellcolor[HTML]{F9CCAD}(19, 19)            & \cellcolor[HTML]{FFE699}455.2           & \cellcolor[HTML]{D5F1A9}2681            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
G-10                                   & (100, 500)                                  & \cellcolor[HTML]{F8CBAD}(17, 17)             & \cellcolor[HTML]{FFE699}865.7          & \cellcolor[HTML]{D5F1A9}1885            & \cellcolor[HTML]{F9CCAD}(15, 15)             & \cellcolor[HTML]{FFE699}384.4          & \cellcolor[HTML]{D5F1A9}110            & \cellcolor[HTML]{F9CCAD}(9, 9)               & \cellcolor[HTML]{FFE699}463.7         & \cellcolor[HTML]{D5F1A9}753            & \cellcolor[HTML]{F9CCAD}(5, 5)               & \cellcolor[HTML]{FFE699}69.6          & \cellcolor[HTML]{D5F1A9}489            & \cellcolor[HTML]{F9CCAD}(5, 5)              & \cellcolor[HTML]{FFE699}164.4          & \cellcolor[HTML]{D5F1A9}139            & \cellcolor[HTML]{F9CCAD}(12, 12)            & \cellcolor[HTML]{FFE699}277.9           & \cellcolor[HTML]{D5F1A9}2409            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
\textbf{Avg.}                              & \textbf{(92, 383)}                          & \cellcolor[HTML]{F8CBAD}\textbf{(17, 18.5)}  & \cellcolor[HTML]{FFE699}\textbf{959.1} & \cellcolor[HTML]{D5F1A9}\textbf{1776.1} & \cellcolor[HTML]{F9CCAD}\textbf{(13.9, 15)}  & \cellcolor[HTML]{FFE699}\textbf{531.1} & \cellcolor[HTML]{D5F1A9}\textbf{110.4} & \cellcolor[HTML]{F9CCAD}\textbf{(9.4, 9.9)}  & \cellcolor[HTML]{FFE699}\textbf{454}  & \cellcolor[HTML]{D5F1A9}\textbf{595.9} & \cellcolor[HTML]{F9CCAD}\textbf{(6.2, 7.1)}  & \cellcolor[HTML]{FFE699}\textbf{130}  & \cellcolor[HTML]{D5F1A9}\textbf{408.4} & \cellcolor[HTML]{F9CCAD}\textbf{(5.7, 6.3)} & \cellcolor[HTML]{FFE699}\textbf{145.2} & \cellcolor[HTML]{D5F1A9}\textbf{106.1} & \cellcolor[HTML]{F9CCAD}\textbf{(22, 18.3)} & \cellcolor[HTML]{FFE699}\textbf{465.6}  & \cellcolor[HTML]{D5F1A9}\textbf{2325.4} & \cellcolor[HTML]{F9CCAD}\textbf{-}    & \cellcolor[HTML]{FFE699}\textbf{-}    & \cellcolor[HTML]{D5F1A9}\textbf{-}    \\ \hline
DL-1                                   & (67, 113)                                   & \cellcolor[HTML]{F8CBAD}(58, 99)             & \cellcolor[HTML]{FFE699}1.4            & \cellcolor[HTML]{D5F1A9}9               & \cellcolor[HTML]{F9CCAD}(10, 13)             & \cellcolor[HTML]{FFE699}5.8            & \cellcolor[HTML]{D5F1A9}33             & \cellcolor[HTML]{F9CCAD}(10, 13)             & \cellcolor[HTML]{FFE699}2.5           & \cellcolor[HTML]{D5F1A9}48             & \cellcolor[HTML]{F9CCAD}(10, 13)             & \cellcolor[HTML]{FFE699}2.5           & \cellcolor[HTML]{D5F1A9}48             & \cellcolor[HTML]{F9CCAD}(10, 13)            & \cellcolor[HTML]{FFE699}2              & \cellcolor[HTML]{D5F1A9}33             & \cellcolor[HTML]{F9CCAD}(22, 32)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}9547            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-2                                   & (59, 97)                                    & \cellcolor[HTML]{F8CBAD}(58, 95)             & \cellcolor[HTML]{FFE699}1.3            & \cellcolor[HTML]{D5F1A9}28              & \cellcolor[HTML]{F9CCAD}(15, 27)             & \cellcolor[HTML]{FFE699}95.5           & \cellcolor[HTML]{D5F1A9}97             & \cellcolor[HTML]{F9CCAD}(11, 19)             & \cellcolor[HTML]{FFE699}45.6          & \cellcolor[HTML]{D5F1A9}106            & \cellcolor[HTML]{F9CCAD}(15, 27)             & \cellcolor[HTML]{FFE699}80.3          & \cellcolor[HTML]{D5F1A9}68             & \cellcolor[HTML]{F9CCAD}(11, 19)            & \cellcolor[HTML]{FFE699}79.8           & \cellcolor[HTML]{D5F1A9}75             & \cellcolor[HTML]{F9CCAD}(17, 31)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7931            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-3                                   & (101, 185)                                  & \cellcolor[HTML]{F8CBAD}(94, 158)            & \cellcolor[HTML]{FFE699}4.7            & \cellcolor[HTML]{D5F1A9}53              & \cellcolor[HTML]{F9CCAD}(6, 9)               & \cellcolor[HTML]{FFE699}10.3           & \cellcolor[HTML]{D5F1A9}30             & \cellcolor[HTML]{F9CCAD}(6, 9)               & \cellcolor[HTML]{FFE699}41.6          & \cellcolor[HTML]{D5F1A9}42             & \cellcolor[HTML]{F9CCAD}(6, 9)               & \cellcolor[HTML]{FFE699}7.8           & \cellcolor[HTML]{D5F1A9}42             & \cellcolor[HTML]{F9CCAD}(6, 9)              & \cellcolor[HTML]{FFE699}26             & \cellcolor[HTML]{D5F1A9}30             & \cellcolor[HTML]{F9CCAD}(12, 22)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}8434            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-4                                   & (47, 85)                                    & \cellcolor[HTML]{F8CBAD}(45, 77)             & \cellcolor[HTML]{FFE699}1              & \cellcolor[HTML]{D5F1A9}18              & \cellcolor[HTML]{F9CCAD}(9, 14)              & \cellcolor[HTML]{FFE699}15.4           & \cellcolor[HTML]{D5F1A9}41             & \cellcolor[HTML]{F9CCAD}(7, 11)              & \cellcolor[HTML]{FFE699}25.9          & \cellcolor[HTML]{D5F1A9}43             & \cellcolor[HTML]{F9CCAD}(9, 14)              & \cellcolor[HTML]{FFE699}15.3          & \cellcolor[HTML]{D5F1A9}38             & \cellcolor[HTML]{F9CCAD}(7, 11)             & \cellcolor[HTML]{FFE699}19.7           & \cellcolor[HTML]{D5F1A9}32             & \cellcolor[HTML]{F9CCAD}(18, 33)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7650            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-5                                   & (35, 55)                                    & \cellcolor[HTML]{F8CBAD}(29, 48)             & \cellcolor[HTML]{FFE699}0.8            & \cellcolor[HTML]{D5F1A9}7               & \cellcolor[HTML]{F9CCAD}(11, 19)             & \cellcolor[HTML]{FFE699}29             & \cellcolor[HTML]{D5F1A9}62             & \cellcolor[HTML]{F9CCAD}(8, 13)              & \cellcolor[HTML]{FFE699}37.5          & \cellcolor[HTML]{D5F1A9}65             & \cellcolor[HTML]{F9CCAD}(11, 19)             & \cellcolor[HTML]{FFE699}33.7          & \cellcolor[HTML]{D5F1A9}35             & \cellcolor[HTML]{F9CCAD}(8, 13)             & \cellcolor[HTML]{FFE699}34.5           & \cellcolor[HTML]{D5F1A9}36             & \cellcolor[HTML]{F9CCAD}(11, 19)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7824            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-6                                   & (126, 246)                                  & \cellcolor[HTML]{F8CBAD}(124, 234)           & \cellcolor[HTML]{FFE699}3.3            & \cellcolor[HTML]{D5F1A9}13              & \cellcolor[HTML]{F9CCAD}(19, 35)             & \cellcolor[HTML]{FFE699}39.4           & \cellcolor[HTML]{D5F1A9}114            & \cellcolor[HTML]{F9CCAD}(7, 12)              & \cellcolor[HTML]{FFE699}2.7           & \cellcolor[HTML]{D5F1A9}134            & \cellcolor[HTML]{F9CCAD}(20, 36)             & \cellcolor[HTML]{FFE699}50.5          & \cellcolor[HTML]{D5F1A9}45             & \cellcolor[HTML]{F9CCAD}(8, 13)             & \cellcolor[HTML]{FFE699}2.4            & \cellcolor[HTML]{D5F1A9}40             & \cellcolor[HTML]{F9CCAD}(25, 46)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}6946            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-7                                   & (108, 207)                                  & \cellcolor[HTML]{F8CBAD}(106, 189)           & \cellcolor[HTML]{FFE699}3.4            & \cellcolor[HTML]{D5F1A9}12              & \cellcolor[HTML]{F9CCAD}(10, 16)             & \cellcolor[HTML]{FFE699}28.3           & \cellcolor[HTML]{D5F1A9}70             & \cellcolor[HTML]{F9CCAD}(6, 9)               & \cellcolor[HTML]{FFE699}26.6          & \cellcolor[HTML]{D5F1A9}67             & \cellcolor[HTML]{F9CCAD}(10, 16)             & \cellcolor[HTML]{FFE699}31.6          & \cellcolor[HTML]{D5F1A9}40             & \cellcolor[HTML]{F9CCAD}(6, 9)              & \cellcolor[HTML]{FFE699}24.7           & \cellcolor[HTML]{D5F1A9}32             & \cellcolor[HTML]{F9CCAD}(28, 42)            & \cellcolor[HTML]{FFE699}2377            & \cellcolor[HTML]{D5F1A9}4767            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-8                                   & (45, 105)                                   & \cellcolor[HTML]{F8CBAD}(39, 75)             & \cellcolor[HTML]{FFE699}1.5            & \cellcolor[HTML]{D5F1A9}13              & \cellcolor[HTML]{F9CCAD}(8, 15)              & \cellcolor[HTML]{FFE699}13.5           & \cellcolor[HTML]{D5F1A9}41             & \cellcolor[HTML]{F9CCAD}(6, 10)              & \cellcolor[HTML]{FFE699}21.4          & \cellcolor[HTML]{D5F1A9}72             & \cellcolor[HTML]{F9CCAD}(9, 17)              & \cellcolor[HTML]{FFE699}7.2           & \cellcolor[HTML]{D5F1A9}38             & \cellcolor[HTML]{F9CCAD}(6, 10)             & \cellcolor[HTML]{FFE699}13.1           & \cellcolor[HTML]{D5F1A9}25             & \cellcolor[HTML]{F9CCAD}(8, 14)             & \cellcolor[HTML]{FFE699}2680            & \cellcolor[HTML]{D5F1A9}6154            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-9                                   & (99, 203)                                   & \cellcolor[HTML]{F8CBAD}(94, 166)            & \cellcolor[HTML]{FFE699}3.5            & \cellcolor[HTML]{D5F1A9}18              & \cellcolor[HTML]{F9CCAD}(10, 16)             & \cellcolor[HTML]{FFE699}9.4            & \cellcolor[HTML]{D5F1A9}41             & \cellcolor[HTML]{F9CCAD}(9, 16)              & \cellcolor[HTML]{FFE699}13            & \cellcolor[HTML]{D5F1A9}44             & \cellcolor[HTML]{F9CCAD}(10, 16)             & \cellcolor[HTML]{FFE699}10.8          & \cellcolor[HTML]{D5F1A9}46             & \cellcolor[HTML]{F9CCAD}(10, 16)            & \cellcolor[HTML]{FFE699}9.8            & \cellcolor[HTML]{D5F1A9}37             & \cellcolor[HTML]{F9CCAD}(17, 26)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7515            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-10                                  & (117, 255)                                  & \cellcolor[HTML]{F8CBAD}(107, 206)           & \cellcolor[HTML]{FFE699}9.9            & \cellcolor[HTML]{D5F1A9}73              & \cellcolor[HTML]{F9CCAD}(5, 9)               & \cellcolor[HTML]{FFE699}11.1           & \cellcolor[HTML]{D5F1A9}44             & \cellcolor[HTML]{F9CCAD}(5, 7)               & \cellcolor[HTML]{FFE699}28.3          & \cellcolor[HTML]{D5F1A9}40             & \cellcolor[HTML]{F9CCAD}(5, 9)               & \cellcolor[HTML]{FFE699}13.7          & \cellcolor[HTML]{D5F1A9}42             & \cellcolor[HTML]{F9CCAD}(5, 7)              & \cellcolor[HTML]{FFE699}27.7           & \cellcolor[HTML]{D5F1A9}44             & \cellcolor[HTML]{F9CCAD}(13, 25)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7202            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-11                                  & (54, 89)                                    & \cellcolor[HTML]{F8CBAD}(51, 84)             & \cellcolor[HTML]{FFE699}0.8            & \cellcolor[HTML]{D5F1A9}5               & \cellcolor[HTML]{F9CCAD}(10, 18)             & \cellcolor[HTML]{FFE699}20.5           & \cellcolor[HTML]{D5F1A9}68             & \cellcolor[HTML]{F9CCAD}(5, 9)               & \cellcolor[HTML]{FFE699}10.1          & \cellcolor[HTML]{D5F1A9}87             & \cellcolor[HTML]{F9CCAD}(10, 19)             & \cellcolor[HTML]{FFE699}29.1          & \cellcolor[HTML]{D5F1A9}37             & \cellcolor[HTML]{F9CCAD}(5, 10)             & \cellcolor[HTML]{FFE699}4.7            & \cellcolor[HTML]{D5F1A9}16             & \cellcolor[HTML]{F9CCAD}(16, 29)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}6587            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-12                                  & (114, 229)                                  & \cellcolor[HTML]{F8CBAD}(111, 204)           & \cellcolor[HTML]{FFE699}4.3            & \cellcolor[HTML]{D5F1A9}27              & \cellcolor[HTML]{F9CCAD}(5, 8)               & \cellcolor[HTML]{FFE699}12.6           & \cellcolor[HTML]{D5F1A9}41             & \cellcolor[HTML]{F9CCAD}(10, 18)             & \cellcolor[HTML]{FFE699}24.1          & \cellcolor[HTML]{D5F1A9}42             & \cellcolor[HTML]{F9CCAD}(5, 8)               & \cellcolor[HTML]{FFE699}15.2          & \cellcolor[HTML]{D5F1A9}66             & \cellcolor[HTML]{F9CCAD}(2, 2)              & \cellcolor[HTML]{FFE699}1.1            & \cellcolor[HTML]{D5F1A9}11             & \cellcolor[HTML]{F9CCAD}(32, 59)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7844            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-13                                  & (94, 171)                                   & \cellcolor[HTML]{F8CBAD}(86, 150)            & \cellcolor[HTML]{FFE699}2.6            & \cellcolor[HTML]{D5F1A9}12              & \cellcolor[HTML]{F9CCAD}(17, 34)             & \cellcolor[HTML]{FFE699}28.3           & \cellcolor[HTML]{D5F1A9}59             & \cellcolor[HTML]{F9CCAD}(9, 17)              & \cellcolor[HTML]{FFE699}30.2          & \cellcolor[HTML]{D5F1A9}167            & \cellcolor[HTML]{F9CCAD}(15, 28)             & \cellcolor[HTML]{FFE699}7.6           & \cellcolor[HTML]{D5F1A9}61             & \cellcolor[HTML]{F9CCAD}(5, 7)              & \cellcolor[HTML]{FFE699}3.4            & \cellcolor[HTML]{D5F1A9}12             & \cellcolor[HTML]{F9CCAD}(19, 31)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}8400            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-14                                  & (53, 109)                                   & \cellcolor[HTML]{F8CBAD}(52, 106)            & \cellcolor[HTML]{FFE699}1.1            & \cellcolor[HTML]{D5F1A9}6               & \cellcolor[HTML]{F9CCAD}(10, 18)             & \cellcolor[HTML]{FFE699}31.2           & \cellcolor[HTML]{D5F1A9}71             & \cellcolor[HTML]{F9CCAD}(7, 13)              & \cellcolor[HTML]{FFE699}45.4          & \cellcolor[HTML]{D5F1A9}78             & \cellcolor[HTML]{F9CCAD}(10, 18)             & \cellcolor[HTML]{FFE699}46.7          & \cellcolor[HTML]{D5F1A9}60             & \cellcolor[HTML]{F9CCAD}(7, 13)             & \cellcolor[HTML]{FFE699}37             & \cellcolor[HTML]{D5F1A9}57             & \cellcolor[HTML]{F9CCAD}(15, 30)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7684            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-15                                  & (114, 202)                                  & \cellcolor[HTML]{F8CBAD}(110, 187)           & \cellcolor[HTML]{FFE699}2.6            & \cellcolor[HTML]{D5F1A9}31              & \cellcolor[HTML]{F9CCAD}(6, 10)              & \cellcolor[HTML]{FFE699}5              & \cellcolor[HTML]{D5F1A9}27             & \cellcolor[HTML]{F9CCAD}(4, 6)               & \cellcolor[HTML]{FFE699}1.4           & \cellcolor[HTML]{D5F1A9}38             & \cellcolor[HTML]{F9CCAD}(6, 10)              & \cellcolor[HTML]{FFE699}2.5           & \cellcolor[HTML]{D5F1A9}26             & \cellcolor[HTML]{F9CCAD}(4, 6)              & \cellcolor[HTML]{FFE699}0.9            & \cellcolor[HTML]{D5F1A9}20             & \cellcolor[HTML]{F9CCAD}(16, 30)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7881            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-16                                  & (110, 184)                                  & \cellcolor[HTML]{F8CBAD}(105, 172)           & \cellcolor[HTML]{FFE699}2.4            & \cellcolor[HTML]{D5F1A9}34              & \cellcolor[HTML]{F9CCAD}(11, 17)             & \cellcolor[HTML]{FFE699}2.9            & \cellcolor[HTML]{D5F1A9}23             & \cellcolor[HTML]{F9CCAD}(10, 15)             & \cellcolor[HTML]{FFE699}3             & \cellcolor[HTML]{D5F1A9}31             & \cellcolor[HTML]{F9CCAD}(11, 17)             & \cellcolor[HTML]{FFE699}2.8           & \cellcolor[HTML]{D5F1A9}29             & \cellcolor[HTML]{F9CCAD}(10, 15)            & \cellcolor[HTML]{FFE699}1.5            & \cellcolor[HTML]{D5F1A9}21             & \cellcolor[HTML]{F9CCAD}(12, 19)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}8172            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-17                                  & (90, 165)                                   & \cellcolor[HTML]{F8CBAD}(88, 149)            & \cellcolor[HTML]{FFE699}2              & \cellcolor[HTML]{D5F1A9}30              & \cellcolor[HTML]{F9CCAD}(6, 13)              & \cellcolor[HTML]{FFE699}4.7            & \cellcolor[HTML]{D5F1A9}29             & \cellcolor[HTML]{F9CCAD}(5, 11)              & \cellcolor[HTML]{FFE699}11.2          & \cellcolor[HTML]{D5F1A9}60             & \cellcolor[HTML]{F9CCAD}(6, 14)              & \cellcolor[HTML]{FFE699}2.9           & \cellcolor[HTML]{D5F1A9}48             & \cellcolor[HTML]{F9CCAD}(5, 12)             & \cellcolor[HTML]{FFE699}5.5            & \cellcolor[HTML]{D5F1A9}26             & \cellcolor[HTML]{F9CCAD}(8, 15)             & \cellcolor[HTML]{FFE699}2646            & \cellcolor[HTML]{D5F1A9}6107            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-18                                  & (44, 92)                                    & \cellcolor[HTML]{F8CBAD}(42, 79)             & \cellcolor[HTML]{FFE699}0.8            & \cellcolor[HTML]{D5F1A9}19              & \cellcolor[HTML]{F9CCAD}(12, 20)             & \cellcolor[HTML]{FFE699}21.2           & \cellcolor[HTML]{D5F1A9}73             & \cellcolor[HTML]{F9CCAD}(3, 3)               & \cellcolor[HTML]{FFE699}0.2           & \cellcolor[HTML]{D5F1A9}69             & \cellcolor[HTML]{F9CCAD}(12, 20)             & \cellcolor[HTML]{FFE699}26.7          & \cellcolor[HTML]{D5F1A9}8              & \cellcolor[HTML]{F9CCAD}(3, 3)              & \cellcolor[HTML]{FFE699}0.8            & \cellcolor[HTML]{D5F1A9}10             & \cellcolor[HTML]{F9CCAD}(18, 30)            & \cellcolor[HTML]{FFE699}1761            & \cellcolor[HTML]{D5F1A9}3985            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-19                                  & (128, 244)                                  & \cellcolor[HTML]{F8CBAD}(125, 209)           & \cellcolor[HTML]{FFE699}3.2            & \cellcolor[HTML]{D5F1A9}24              & \cellcolor[HTML]{F9CCAD}(3, 3)               & \cellcolor[HTML]{FFE699}0.6            & \cellcolor[HTML]{D5F1A9}12             & \cellcolor[HTML]{F9CCAD}(3, 3)               & \cellcolor[HTML]{FFE699}0.7           & \cellcolor[HTML]{D5F1A9}14             & \cellcolor[HTML]{F9CCAD}(3, 3)               & \cellcolor[HTML]{FFE699}0.5           & \cellcolor[HTML]{D5F1A9}12             & \cellcolor[HTML]{F9CCAD}(3, 3)              & \cellcolor[HTML]{FFE699}1.3            & \cellcolor[HTML]{D5F1A9}12             & \cellcolor[HTML]{F9CCAD}(5, 5)              & \cellcolor[HTML]{FFE699}2608            & \cellcolor[HTML]{D5F1A9}5433            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
DL-20                                  & (80, 164)                                   & \cellcolor[HTML]{F8CBAD}(75, 131)            & \cellcolor[HTML]{FFE699}1.4            & \cellcolor[HTML]{D5F1A9}17              & \cellcolor[HTML]{F9CCAD}(6, 9)               & \cellcolor[HTML]{FFE699}15.3           & \cellcolor[HTML]{D5F1A9}21             & \cellcolor[HTML]{F9CCAD}(3, 3)               & \cellcolor[HTML]{FFE699}0.3           & \cellcolor[HTML]{D5F1A9}32             & \cellcolor[HTML]{F9CCAD}(6, 9)               & \cellcolor[HTML]{FFE699}8.8           & \cellcolor[HTML]{D5F1A9}11             & \cellcolor[HTML]{F9CCAD}(3, 3)              & \cellcolor[HTML]{FFE699}0.2            & \cellcolor[HTML]{D5F1A9}9              & \cellcolor[HTML]{F9CCAD}(27, 42)            & \cellcolor[HTML]{FFE699}3600*            & \cellcolor[HTML]{D5F1A9}7775            & \cellcolor[HTML]{F9CCAD}-             & \cellcolor[HTML]{FFE699}-             & \cellcolor[HTML]{D5F1A9}-             \\
\textbf{Avg.}                              & \textbf{(84.3, 160)}                        & \cellcolor[HTML]{F8CBAD}\textbf{(80, 140.9)} & \cellcolor[HTML]{FFE699}\textbf{2.6}   & \cellcolor[HTML]{D5F1A9}\textbf{22.5}   & \cellcolor[HTML]{F9CCAD}\textbf{(9.5, 16.2)} & \cellcolor[HTML]{FFE699}\textbf{20}    & \cellcolor[HTML]{D5F1A9}\textbf{49.9}  & \cellcolor[HTML]{F9CCAD}\textbf{(6.7, 10.9)} & \cellcolor[HTML]{FFE699}\textbf{18.6} & \cellcolor[HTML]{D5F1A9}\textbf{64}    & \cellcolor[HTML]{F9CCAD}\textbf{(9.5, 16.1)} & \cellcolor[HTML]{FFE699}\textbf{19.8} & \cellcolor[HTML]{D5F1A9}\textbf{40}    & \cellcolor[HTML]{F9CCAD}\textbf{(6.2, 9.7)} & \cellcolor[HTML]{FFE699}\textbf{14.8}  & \cellcolor[HTML]{D5F1A9}\textbf{28.9}  & \cellcolor[HTML]{F9CCAD}\textbf{(17, 29)}   & \cellcolor[HTML]{FFE699}\textbf{3303.6} & \cellcolor[HTML]{D5F1A9}\textbf{7191.9} & \cellcolor[HTML]{F9CCAD}\textbf{-}    & \cellcolor[HTML]{FFE699}\textbf{-}    & \cellcolor[HTML]{D5F1A9}\textbf{-}    \\ \hline
JS-1                                   & 134                                         & \cellcolor[HTML]{F8CBAD}64                   & \cellcolor[HTML]{FFE699}72             & \cellcolor[HTML]{D5F1A9}114             & \cellcolor[HTML]{F9CCAD}83                   & \cellcolor[HTML]{FFE699}141.5          & \cellcolor[HTML]{D5F1A9}172            & \cellcolor[HTML]{F9CCAD}20                   & \cellcolor[HTML]{FFE699}35.4          & \cellcolor[HTML]{D5F1A9}351            & \cellcolor[HTML]{F9CCAD}86                   & \cellcolor[HTML]{FFE699}79.9          & \cellcolor[HTML]{D5F1A9}73             & \cellcolor[HTML]{F9CCAD}20                  & \cellcolor[HTML]{FFE699}23.6           & \cellcolor[HTML]{D5F1A9}40             & \cellcolor[HTML]{F9CCAD}25                  & \cellcolor[HTML]{FFE699}16.5            & \cellcolor[HTML]{D5F1A9}30              & \cellcolor[HTML]{F9CCAD}34            & \cellcolor[HTML]{FFE699}2.1           & \cellcolor[HTML]{D5F1A9}4             \\
JS-2                                   & 508                                         & \cellcolor[HTML]{F8CBAD}170                  & \cellcolor[HTML]{FFE699}505.2          & \cellcolor[HTML]{D5F1A9}686             & \cellcolor[HTML]{F9CCAD}142                  & \cellcolor[HTML]{FFE699}236.8          & \cellcolor[HTML]{D5F1A9}178            & \cellcolor[HTML]{F9CCAD}70                   & \cellcolor[HTML]{FFE699}143.5         & \cellcolor[HTML]{D5F1A9}414            & \cellcolor[HTML]{F9CCAD}146                  & \cellcolor[HTML]{FFE699}115.4         & \cellcolor[HTML]{D5F1A9}268            & \cellcolor[HTML]{F9CCAD}64                  & \cellcolor[HTML]{FFE699}52.9           & \cellcolor[HTML]{D5F1A9}86             & \cellcolor[HTML]{F9CCAD}86                  & \cellcolor[HTML]{FFE699}80.5            & \cellcolor[HTML]{D5F1A9}125             & \cellcolor[HTML]{F9CCAD}97            & \cellcolor[HTML]{FFE699}28.9          & \cellcolor[HTML]{D5F1A9}47            \\
JS-3                                   & 182                                         & \cellcolor[HTML]{F8CBAD}34                   & \cellcolor[HTML]{FFE699}66.9           & \cellcolor[HTML]{D5F1A9}114             & \cellcolor[HTML]{F9CCAD}20                   & \cellcolor[HTML]{FFE699}42.4           & \cellcolor[HTML]{D5F1A9}40             & \cellcolor[HTML]{F9CCAD}11                   & \cellcolor[HTML]{FFE699}29            & \cellcolor[HTML]{D5F1A9}76             & \cellcolor[HTML]{F9CCAD}20                   & \cellcolor[HTML]{FFE699}24.6          & \cellcolor[HTML]{D5F1A9}54             & \cellcolor[HTML]{F9CCAD}19                  & \cellcolor[HTML]{FFE699}19.4           & \cellcolor[HTML]{D5F1A9}33             & \cellcolor[HTML]{F9CCAD}15                  & \cellcolor[HTML]{FFE699}14.6            & \cellcolor[HTML]{D5F1A9}26              & \cellcolor[HTML]{F9CCAD}15            & \cellcolor[HTML]{FFE699}11.7          & \cellcolor[HTML]{D5F1A9}19            \\
JS-4                                   & 264                                         & \cellcolor[HTML]{F8CBAD}33                   & \cellcolor[HTML]{FFE699}44.5           & \cellcolor[HTML]{D5F1A9}78              & \cellcolor[HTML]{F9CCAD}34                   & \cellcolor[HTML]{FFE699}86.2           & \cellcolor[HTML]{D5F1A9}82             & \cellcolor[HTML]{F9CCAD}7                    & \cellcolor[HTML]{FFE699}57.6          & \cellcolor[HTML]{D5F1A9}192            & \cellcolor[HTML]{F9CCAD}34                   & \cellcolor[HTML]{FFE699}39.5          & \cellcolor[HTML]{D5F1A9}118            & \cellcolor[HTML]{F9CCAD}7                   & \cellcolor[HTML]{FFE699}15.8           & \cellcolor[HTML]{D5F1A9}29             & \cellcolor[HTML]{F9CCAD}18                  & \cellcolor[HTML]{FFE699}22.4            & \cellcolor[HTML]{D5F1A9}41              & \cellcolor[HTML]{F9CCAD}25            & \cellcolor[HTML]{FFE699}7.6           & \cellcolor[HTML]{D5F1A9}12            \\
JS-5                                   & 347                                         & \cellcolor[HTML]{F8CBAD}81                   & \cellcolor[HTML]{FFE699}115.3          & \cellcolor[HTML]{D5F1A9}185             & \cellcolor[HTML]{F9CCAD}57                   & \cellcolor[HTML]{FFE699}140.3          & \cellcolor[HTML]{D5F1A9}73             & \cellcolor[HTML]{F9CCAD}43                   & \cellcolor[HTML]{FFE699}125.3         & \cellcolor[HTML]{D5F1A9}242            & \cellcolor[HTML]{F9CCAD}66                   & \cellcolor[HTML]{FFE699}47            & \cellcolor[HTML]{D5F1A9}207            & \cellcolor[HTML]{F9CCAD}43                  & \cellcolor[HTML]{FFE699}26.9           & \cellcolor[HTML]{D5F1A9}43             & \cellcolor[HTML]{F9CCAD}52                  & \cellcolor[HTML]{FFE699}44.2            & \cellcolor[HTML]{D5F1A9}81              & \cellcolor[HTML]{F9CCAD}38            & \cellcolor[HTML]{FFE699}31.7          & \cellcolor[HTML]{D5F1A9}47            \\
JS-6                                   & 131                                         & \cellcolor[HTML]{F8CBAD}41                   & \cellcolor[HTML]{FFE699}42.6           & \cellcolor[HTML]{D5F1A9}74              & \cellcolor[HTML]{F9CCAD}34                   & \cellcolor[HTML]{FFE699}60.6           & \cellcolor[HTML]{D5F1A9}34             & \cellcolor[HTML]{F9CCAD}17                   & \cellcolor[HTML]{FFE699}41.7          & \cellcolor[HTML]{D5F1A9}99             & \cellcolor[HTML]{F9CCAD}34                   & \cellcolor[HTML]{FFE699}21.7          & \cellcolor[HTML]{D5F1A9}76             & \cellcolor[HTML]{F9CCAD}19                  & \cellcolor[HTML]{FFE699}17.4           & \cellcolor[HTML]{D5F1A9}28             & \cellcolor[HTML]{F9CCAD}27                  & \cellcolor[HTML]{FFE699}21.9            & \cellcolor[HTML]{D5F1A9}38              & \cellcolor[HTML]{F9CCAD}36            & \cellcolor[HTML]{FFE699}12.4          & \cellcolor[HTML]{D5F1A9}21            \\
JS-7                                   & 246                                         & \cellcolor[HTML]{F8CBAD}40                   & \cellcolor[HTML]{FFE699}36.8           & \cellcolor[HTML]{D5F1A9}64              & \cellcolor[HTML]{F9CCAD}24                   & \cellcolor[HTML]{FFE699}63.4           & \cellcolor[HTML]{D5F1A9}51             & \cellcolor[HTML]{F9CCAD}13                   & \cellcolor[HTML]{FFE699}50.6          & \cellcolor[HTML]{D5F1A9}122            & \cellcolor[HTML]{F9CCAD}24                   & \cellcolor[HTML]{FFE699}27.9          & \cellcolor[HTML]{D5F1A9}107            & \cellcolor[HTML]{F9CCAD}13                  & \cellcolor[HTML]{FFE699}15.2           & \cellcolor[HTML]{D5F1A9}28             & \cellcolor[HTML]{F9CCAD}19                  & \cellcolor[HTML]{FFE699}23.5            & \cellcolor[HTML]{D5F1A9}43              & \cellcolor[HTML]{F9CCAD}30            & \cellcolor[HTML]{FFE699}9.6           & \cellcolor[HTML]{D5F1A9}17            \\
JS-8                                   & 549                                         & \cellcolor[HTML]{F8CBAD}134                  & \cellcolor[HTML]{FFE699}175.6          & \cellcolor[HTML]{D5F1A9}298             & \cellcolor[HTML]{F9CCAD}131                  & \cellcolor[HTML]{FFE699}433.8          & \cellcolor[HTML]{D5F1A9}310            & \cellcolor[HTML]{F9CCAD}77                   & \cellcolor[HTML]{FFE699}208.8         & \cellcolor[HTML]{D5F1A9}694            & \cellcolor[HTML]{F9CCAD}163                  & \cellcolor[HTML]{FFE699}165.1         & \cellcolor[HTML]{D5F1A9}347            & \cellcolor[HTML]{F9CCAD}103                 & \cellcolor[HTML]{FFE699}87.8           & \cellcolor[HTML]{D5F1A9}136            & \cellcolor[HTML]{F9CCAD}102                 & \cellcolor[HTML]{FFE699}73.5            & \cellcolor[HTML]{D5F1A9}128             & \cellcolor[HTML]{F9CCAD}103           & \cellcolor[HTML]{FFE699}28.6          & \cellcolor[HTML]{D5F1A9}45            \\
JS-9                                   & 144                                         & \cellcolor[HTML]{F8CBAD}20                   & \cellcolor[HTML]{FFE699}10.5           & \cellcolor[HTML]{D5F1A9}20              & \cellcolor[HTML]{F9CCAD}19                   & \cellcolor[HTML]{FFE699}76             & \cellcolor[HTML]{D5F1A9}311            & \cellcolor[HTML]{F9CCAD}7                    & \cellcolor[HTML]{FFE699}41.5          & \cellcolor[HTML]{D5F1A9}104            & \cellcolor[HTML]{F9CCAD}23                   & \cellcolor[HTML]{FFE699}22.4          & \cellcolor[HTML]{D5F1A9}73             & \cellcolor[HTML]{F9CCAD}7                   & \cellcolor[HTML]{FFE699}10.7           & \cellcolor[HTML]{D5F1A9}20             & \cellcolor[HTML]{F9CCAD}13                  & \cellcolor[HTML]{FFE699}7.6             & \cellcolor[HTML]{D5F1A9}14              & \cellcolor[HTML]{F9CCAD}36            & \cellcolor[HTML]{FFE699}3.8           & \cellcolor[HTML]{D5F1A9}7             \\
JS-10                                  & 569                                         & \cellcolor[HTML]{F8CBAD}28                   & \cellcolor[HTML]{FFE699}18.3           & \cellcolor[HTML]{D5F1A9}34              & \cellcolor[HTML]{F9CCAD}12                   & \cellcolor[HTML]{FFE699}93.5           & \cellcolor[HTML]{D5F1A9}312            & \cellcolor[HTML]{F9CCAD}12                   & \cellcolor[HTML]{FFE699}55.3          & \cellcolor[HTML]{D5F1A9}100            & \cellcolor[HTML]{F9CCAD}12                   & \cellcolor[HTML]{FFE699}11.8          & \cellcolor[HTML]{D5F1A9}100            & \cellcolor[HTML]{F9CCAD}12                  & \cellcolor[HTML]{FFE699}11.4           & \cellcolor[HTML]{D5F1A9}20             & \cellcolor[HTML]{F9CCAD}12                  & \cellcolor[HTML]{FFE699}12              & \cellcolor[HTML]{D5F1A9}23              & \cellcolor[HTML]{F9CCAD}13            & \cellcolor[HTML]{FFE699}8.4           & \cellcolor[HTML]{D5F1A9}15            \\
\textbf{Avg.}                              & \textbf{307.4}                              & \cellcolor[HTML]{F8CBAD}\textbf{64.5}        & \cellcolor[HTML]{FFE699}\textbf{108.8} & \cellcolor[HTML]{D5F1A9}\textbf{166.7}  & \cellcolor[HTML]{F9CCAD}\textbf{55.6}        & \cellcolor[HTML]{FFE699}\textbf{137.5} & \cellcolor[HTML]{D5F1A9}\textbf{156.3} & \cellcolor[HTML]{F9CCAD}\textbf{27.7}        & \cellcolor[HTML]{FFE699}\textbf{78.9} & \cellcolor[HTML]{D5F1A9}\textbf{239.4} & \cellcolor[HTML]{F9CCAD}\textbf{60.8}        & \cellcolor[HTML]{FFE699}\textbf{55.5} & \cellcolor[HTML]{D5F1A9}\textbf{142.3} & \cellcolor[HTML]{F9CCAD}\textbf{30.7}       & \cellcolor[HTML]{FFE699}\textbf{28.1}  & \cellcolor[HTML]{D5F1A9}\textbf{46.3}  & \cellcolor[HTML]{F9CCAD}\textbf{36.9}       & \cellcolor[HTML]{FFE699}\textbf{31.7}   & \cellcolor[HTML]{D5F1A9}\textbf{54.9}   & \cellcolor[HTML]{F9CCAD}\textbf{42.7} & \cellcolor[HTML]{FFE699}\textbf{14.5} & \cellcolor[HTML]{D5F1A9}\textbf{23.4} \\ \hline
\end{tabular}%
}
\end{table*}



==> tables/t1_small.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[h]\scriptsize
\centering
\caption{Detailed Data of Experiment Result}
\label{experiment_result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrr}
\hline
\multicolumn{1}{c}{}                                     & \multicolumn{1}{c}{}                        & \multicolumn{3}{c}{GReduce_{r}}                                                                               & \multicolumn{3}{c}{Greduce^{S}_{b}}                                                                           & \multicolumn{3}{c}{Greduce^{S}_{a}}                                                                           & \multicolumn{3}{c}{Greduce^{T}_{b}}                                                                           & \multicolumn{3}{c}{Greduce^{T}_{a}}                                                                          & \multicolumn{3}{c}{Perses}                                                                                   & \multicolumn{3}{c}{JSDelta}                                                                                   \\
\multicolumn{1}{c}{\multirow{-2}{*}{Application Domain}} & \multicolumn{1}{c}{\multirow{-2}{*}{S_{o}}} & \cellcolor[HTML]{F8CBAD}\textbf{S}  & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} & \cellcolor[HTML]{F9CCAD}\textbf{S}  & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} & \cellcolor[HTML]{F9CCAD}\textbf{S}  & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} & \cellcolor[HTML]{F9CCAD}\textbf{S}  & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} & \cellcolor[HTML]{F9CCAD}\textbf{S} & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} & \cellcolor[HTML]{F9CCAD}\textbf{S} & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} & \cellcolor[HTML]{F9CCAD}\textbf{S} & \cellcolor[HTML]{FFE699}\textbf{T} & \cellcolor[HTML]{D5F1A9}\textbf{P} \\ \hline
Graphs                                                   & (92, 383)                                   & \cellcolor[HTML]{F8CBAD}(17, 18.5)  & \cellcolor[HTML]{FFE699}959.1      & \cellcolor[HTML]{D5F1A9}1776.1     & \cellcolor[HTML]{F9CCAD}(13.9, 15)  & \cellcolor[HTML]{FFE699}531.1      & \cellcolor[HTML]{D5F1A9}110.4      & \cellcolor[HTML]{F9CCAD}(9.4, 9.9)  & \cellcolor[HTML]{FFE699}454        & \cellcolor[HTML]{D5F1A9}595.9      & \cellcolor[HTML]{F9CCAD}(6.2, 7.1)  & \cellcolor[HTML]{FFE699}130        & \cellcolor[HTML]{D5F1A9}408.4      & \cellcolor[HTML]{F9CCAD}(5.7, 6.3) & \cellcolor[HTML]{FFE699}145.2      & \cellcolor[HTML]{D5F1A9}106.1      & \cellcolor[HTML]{F9CCAD}(22, 18.3) & \cellcolor[HTML]{FFE699}465.6      & \cellcolor[HTML]{D5F1A9}2325.4     & \cellcolor[HTML]{F9CCAD}-          & \cellcolor[HTML]{FFE699}-          & \cellcolor[HTML]{D5F1A9}-          \\
DL Models                                                & (84.3, 160)                                 & \cellcolor[HTML]{F8CBAD}(80, 140.9) & \cellcolor[HTML]{FFE699}2.6        & \cellcolor[HTML]{D5F1A9}22.5       & \cellcolor[HTML]{F9CCAD}(9.5, 16.2) & \cellcolor[HTML]{FFE699}20         & \cellcolor[HTML]{D5F1A9}49.9       & \cellcolor[HTML]{F9CCAD}(6.7, 10.9) & \cellcolor[HTML]{FFE699}18.6       & \cellcolor[HTML]{D5F1A9}64         & \cellcolor[HTML]{F9CCAD}(9.5, 16.1) & \cellcolor[HTML]{FFE699}19.8       & \cellcolor[HTML]{D5F1A9}40         & \cellcolor[HTML]{F9CCAD}(6.2, 9.7) & \cellcolor[HTML]{FFE699}14.8       & \cellcolor[HTML]{D5F1A9}28.9       & \cellcolor[HTML]{F9CCAD}(17, 29)   & \cellcolor[HTML]{FFE699}3303.6     & \cellcolor[HTML]{D5F1A9}7191.9     & \cellcolor[HTML]{F9CCAD}-          & \cellcolor[HTML]{FFE699}-          & \cellcolor[HTML]{D5F1A9}-          \\
JS Programs                                              & 307.4                                       & \cellcolor[HTML]{F8CBAD}64.5        & \cellcolor[HTML]{FFE699}108.8      & \cellcolor[HTML]{D5F1A9}166.7      & \cellcolor[HTML]{F9CCAD}55.6        & \cellcolor[HTML]{FFE699}137.5      & \cellcolor[HTML]{D5F1A9}156.3      & \cellcolor[HTML]{F9CCAD}27.7        & \cellcolor[HTML]{FFE699}78.9       & \cellcolor[HTML]{D5F1A9}239.4      & \cellcolor[HTML]{F9CCAD}60.8        & \cellcolor[HTML]{FFE699}55.5       & \cellcolor[HTML]{D5F1A9}142.3      & \cellcolor[HTML]{F9CCAD}30.7       & \cellcolor[HTML]{FFE699}28.1       & \cellcolor[HTML]{D5F1A9}46.3       & \cellcolor[HTML]{F9CCAD}36.9       & \cellcolor[HTML]{FFE699}31.7       & \cellcolor[HTML]{D5F1A9}54.9       & \cellcolor[HTML]{F9CCAD}42.7       & \cellcolor[HTML]{FFE699}14.5       & \cellcolor[HTML]{D5F1A9}23.4       \\ \hline
\end{tabular}%
}
\end{table*}



==> tables/t2.tex <==
% Please a\da the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\caption{The size of reduction results, reduction time, number of property tests and
reduction speeds on average \rev{for graphs, DL models, and JavaScript programs} (the grey columns are ratios of metrics between $G^{\db}_{\ssc}$ and Perses, $G^{\db}_{\ssc}$ and JSDelta, \rev{$G^{\db}_{\ssc}$ and ~\emph{ddmin}}, $G^{\db}_{\ssc}$ and T-PDD).
}
\label{tab:res}

\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|rrrrrrr
>{\columncolor[HTML]{C0C0C0}}r r
>{\columncolor[HTML]{C0C0C0}}r r
>{\columncolor[HTML]{C0C0C0}}r r
>{\columncolor[HTML]{C0C0C0}}r
}
\hline
\multicolumn{1}{c|}{{\color[HTML]{333333} Domains}} & \multicolumn{1}{c|}{{\color[HTML]{333333} Metrics}} & \multicolumn{1}{c}{{\color[HTML]{333333} $G_{h}^{S}$}} & \multicolumn{1}{c}{{\color[HTML]{333333} $G_{b}^{S}$}} & \multicolumn{1}{c}{{\color[HTML]{333333} $G_{r}^{S}$}} & \multicolumn{1}{c}{{\color[HTML]{333333} $G_{h}^{T}$}} & \multicolumn{1}{c}{{\color[HTML]{333333} $G_{b}^{T}$}} & \multicolumn{1}{c}{{\color[HTML]{333333} $G_{r}^{T}$}} & \multicolumn{1}{c}{{\color[HTML]{333333} $Perses$}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0} Ratio } & \multicolumn{1}{c}{{\color[HTML]{333333} $JSDelta$}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0} Ratio} & \multicolumn{1}{c}{{\color[HTML]{333333} \rev{$ddmin$}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0} \rev{Ratio}} & \multicolumn{1}{c}{{\color[HTML]{333333} \rev{$T-PDD$}}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0} \rev{Ratio}}                        \\ \hline
\multicolumn{1}{l|}{}                        & Size                                        & (17.0, 18.3)                                            & (13.9, 15.0)                                            & (9.4, 9.8)                                              & (17.0, 18.3)                                             & (6.2, 7.1)                                               & {\ul \textbf{(5.5, 6.0)}}                                & (22.0, 18.3)                                        & 28.5\%                             & -                                                    & -  & \rev{(26.4, 16.3)} &  \rev{26.9\%}                                                     &      (37.5, 38.2)        &                 \\
\multicolumn{1}{l|}{}                        & Time                                         & 530.7s                                                   & 283.0s                                                   & 237.7s                                                   & 501.3s                                                    & {\ul \textbf{73.2s}}                                      & 81.6s                                                     & 465.6s                                               & 17.5\%                                       & -                                                    & -  & \rev{329.8s} & \rev{24.7\%}                                                      &     588.7s         &                 \\
\multicolumn{1}{l|}{}                        & \#tests                                        & 422.8                                                   & 595.7                                                   & 405.0                                                   & 439.3                                                    & 120.1                                                    & {\ul \textbf{119.2}}                                     & 2325.4                                              & 5.1\%                                        & -                                                    & -    &  \rev{2337.9}  & \rev{5.1\%}                                                  &    1904.5          &                 \\
\multicolumn{1}{l|}{\multirow{-4}{*}{Graphs}} & Speed                                        & 8.2                                                     & 13.8                                                    & 11.8                                                    & 8.1                                                      & {\ul \textbf{19.3}}                                      & 16.3                                                     & 2.3                                                 & 7.2x                                         & -                                                    & -  &  \rev{3.96} & \rev{4.1x}                                                      &     1.4         &                 \\ \hline
\multicolumn{1}{l|}{}                        & Size                                        & (80.0, 140.9)                                           & (9.6, 16.4)                                             & (6.9, 11.1)                                             & (80.0, 141.2)                                            & (9.4, 16.0)                                              & {\ul \textbf{(6.2, 9.7)}}                                & (17.0, 29.0)                                        & 34.6\%                             & -                                                    & -  & \rev{(21.4, 38.4)} &  \rev{26.6\%}                                                     &   (65.5,114.8)           &                 \\
\multicolumn{1}{l|}{}                        & Time                                         & 3.1s                                                     & 24.3s                                                    & 23.8s                                                    & {\ul \textbf{2.2s}}                                       & 23.3s                                                     & 18.4s                                                     & 3303.6s                                              & 0.6\%                                        & -                                                    & -   & \rev{1158.1s} & \rev{1.6\%}                                                     &    3600.0s          &                 \\
\multicolumn{1}{l|}{}                        & \#tests                                        & 21.9                                                    & 61.6                                                    & 38.1                                                    & {\ul \textbf{12.7}}                                      & 51.4                                                     & 28.6                                                     & 7191.9                                              & 0.4\%                                        & -                                                    & - & \rev{5685.0} & \rev{0.5\%}                                                       &    5905.1          &                 \\
\multicolumn{1}{l|}{\multirow{-4}{*}{DL models}}    & Speed                                        & 8.3                                                     & 36.9                                                    & 51.2                                                    & 10.7                                                     & 37.2                                                     & {\ul \textbf{58.7}}                                      & 0.06                                                 & 949.3x                                       & -                                                    & -  & \rev{0.17} & \rev{349.4x}                                                       &      0.02        &                 \\ \hline
\multicolumn{1}{l|}{}                        & Size                                        & 57.5                                                    & 45.8                                                    & 21.8                                                    & 57.5                                                     & 47.8                                                     & {\ul \textbf{21.4}}                                      & 28.3                                                & 75.6\%                                       & 35.3                                                 & 60.6\%  & \rev{-} & \rev{-}                                                 &      25.5        &                 \\
\multicolumn{1}{l|}{}                        & Time                                         & 79.8s                                                    & 91.2s                                                    & 63.6s                                                    & 92.1s                                                     & 36.3s                                                     & {\ul 21.4s}                                               & 32.6s                                                & 65.4\%                                       & \textbf{13.1s}                                        & 162.8\%  & \rev{-} & \rev{-}                                                 &     97.0s         &                 \\
\multicolumn{1}{l|}{}                        & \#tests                                        & 79.5                                                    & 36.8                                                    & 37.5                                                    & 83.3                                                     & 25.4                                                     & {\ul 25.1}                                               & 53.7                                                & 46.7\%                                       & \textbf{21.4}                                        & 117.3\%  & \rev{-} & \rev{-}                                                 &     117.3         &                 \\
\multicolumn{1}{l|}{\multirow{-4}{*}{JS programs}}    & Speed                                        & 7.8                                                     & 3.7                                                     & 4.5                                                     & 5.2                                                      & 12.3                                                     & {\ul 15.9}                                               & 12.1                                                & 1.3x                                         & \textbf{25.4}                                        & 0.6x  & \rev{-} & \rev{-}                                                    &    3.2          &                 \\ \hline

\end{tabular}%
}
\end{table}

==> tables/t2_test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllll}
\multicolumn{2}{l}{\textbf{}}         & \textbf{$G_{r}^{DD}$} & \textbf{$G_{b}^{DD}$} & \textbf{$G_{a}^{DD}$} & \textbf{$G_{r}^{HDD}$} & \textbf{$G_{b}^{HDD}$} & \textbf{$G_{a}^{HDD}$} & \textbf{$Perses$} & \textbf{$JSDelta$} \\
\multirow{4}{*}{Graph}       & size               
\end{tabular}%
}
\end{table}
